Finding equilibria: simpler for pessimists, simplest for optimists

We consider simple stochastic games with terminal-node rewards and multiple players, who have differing perceptions of risk. Specifically, we study risk-sensitive equilibria (RSEs), where no player can improve their perceived reward -- based on their risk parameter -- by deviating from their strategy. We start with the entropic risk (ER) measure, which is widely studied in finance. ER characterises the players on a quantitative spectrum, with positive risk parameters representing optimists and negative parameters representing pessimists. Building on known results for Nash equilibira, we show that RSEs exist under ER for all games with non-negative terminal rewards. However, using similar techniques, we also show that the corresponding constrained existence problem -- to determine whether an RSE exists under ER with the payoffs in given intervals -- is undecidable. To address this, we introduce a new, qualitative risk measure -- called extreme risk (XR) -- which coincides with the limit cases of positively infinite and negatively infinite ER parameters. Under XR, every player is an extremist: an extreme optimist perceives their reward as the maximum payoff that can be achieved with positive probability, while an extreme pessimist expects the minimum payoff achievable with positive probability. Our first main result proves the existence of RSEs also under XR for non-negative terminal rewards. Our second main result shows that under XR the constrained existence problem is not only decidable, but NP-complete. Moreover, when all players are extreme optimists, the problem becomes PTIME-complete. Our algorithmic results apply to all rewards, positive or negative, establishing the first decidable fragment for equilibria in simple stochastic games with terminal objectives without restrictions on strategy types or number of players.

==> 4zExistenceProblem.tex <==
%\leonard{This is only the old proof, and should not appear in the paper.}

% \begin{theorem}[Existence of RSE]
%     Let $\Game_{\|v_0}$ be a multiplayer simple stochastic game with only non-negative rewards, and let $\brho \in \{\pm \infty\}^\Pi$.
%     Then, there exists a stationary strategy that is a $(P,O)$-RSE in $\Game_{\|v_0}$.
%     Moreover, there exists an algorithm that, given such a game, outputs the representation of such an RSE in time $\Oh(m^2 p)$, where $m$ is the number of edge and $p$ is the number of players.
% \end{theorem}

% \begin{proof}
%     \leonard{Should be a functional proof, feel free to check}

%     Let $\Game_{\|v_0}$ be a game, and let  $(P,O)$ represent the partition of the players into pessimists and optimists. 
%     We define a decreasing sequence $E_0, E_1, \dots$ of subsets of $E$, satisfying the invariant that for each $n$, each stochastic vertex has all its outgoing edges in $E_n$, and that each non-stochastic and non-terminal vertex has at least one.


%     First, we define $E_0 = E$, which immediately satisfies the invariant.\theju{invariant. Not induction hyp.}
%     When $E_n$ is defined, let us consider the game $\Game^n_{\|v_0}$ defined as equal to $\Game_{\|v_0}$ but where the edges that do not belong to $E_n$ have been removed (that is indeed a game structure by the invariant).
%     Let us consider the memoryless strategy profile $\bsigma^n$ that consists, from each vertex $v$, in taking with positive probability any edge $vw \in E_n$.
%     If $\bsigma^n$ is an RSE in $\Game_{\|v_0}^n$, we stop there.
%     If it is not, then let $i$ be a player that has a profitable deviation $\sigma'_i$ --- note that we are only considering the game $\Game_{\|v_0}^n$, and that therefore $\sigma'_i$ uses no more edges than $\sigma^n_i$.
%     By TODO, we can assume that $\sigma'_i$ is positional.

%     If player $i$ is optimistic, then there exists a payoff $x$ such that $\prob_{\bsigma^n}(\mu_i = x) = 0$, that $\prob_{\bsigma^n_{-i}, \sigma'_i}(\mu_i = x) > 0$, and that every payoff that player $i$ has positive probability to get in $\bsigma^n$ is strictly smaller than $x$.
%     Moreover, since we assume that all the rewards are positive, we necessarily have $x > 0$.
%     But, in the strategy profile $\bsigma^n$, all the terminal vertices that are accessible from $v_0$ in the game $\Game^n$ are reached with positive probability: that case is therefore impossible.

%     If player $i$ is pessimistic, let $y_n = \X(\bsigma^n)[\mu_i]$.
%     Then, when following the strategy profile $(\bsigma_{-i}^n, \sigma'_i)$, player $i$ gets almost surely more than the payoff $y_n$.
%     Let $W_n$ be the set of vertices $v$ from which whatever player $i$ does, their risk entropy is $y_n$ or less; formally, the set of vertices $v$ such that from $v$, in the game $\Game^n$, for every strategy $\tau_i$ of player $i$, we have $\prob_{\bsigma_{-i}^n, \tau_i}(\mu_i \leq y_n) > 0$.
%     The set $W_n$ is nonempty and accessible from $v_0$ in $(V, E_n)$.
%     Indeed, if $y_n$ is obtained by reaching a terminal vertex $t$, then we have $t \in W_n$, and $t$ is accessible from $v_0$.
%     If now $y_n = 0$ is obtained by reaching no terminal vertex, then when following $\bsigma^n$, with positive probability, no terminal is reached.
%     Then, there is in particular a vertex $u$ that has positive probability to be visited infinitely often.
%     And when playing $\bsigma^n$ from $u$, the probability that some terminal is ever reached is actually $0$, since if it was some constant $q > 0$, then the probability of visiting it infinitely often would be $\lim_k (1-q)^k = 0$.
%     In other words, no terminal vertex is accessible from $u$ in $(V, E_n)$, hence $u \in W_n$.

%     Now, let us note that since $\sigma'_i$ is a profitable deviation, we have $v_0 \not\in W_n$, and since $W_n$ is nonempty and accessible from $v_0$, there exists at least one edge $vw \in E_n$ such that $v \not\in W_n$ and $w \in W_n$.
%     For each such edge, we have $v \in V_i$, and there exists at least one other edge $vw' \in E_n$ with $w' \not\in W_n$: otherwise, for every strategy $\tau_i$ of player $i$, the strategy profile $(\btau^n_{-i}, \tau_i)$, played from $v$, would with positive probability reach the vertex $w$ and then give player $i$ the payoff $y_n$, which contradicts the fact that $v \not\in W_n$.
%     We can therefore define $E_{n+1} \subseteq E_n$ by removing all such edges and only them: the invariant still holds (TODO: check).

%     Now, since there is at least one vertex that is removed at each step, the sequence is necessarily finite: there is $n$ such that $\bsigma^n$ is an RSE in $\Game^n_{\|v_0}$.
%     Let us prove that it is also an RSE in $\Game_{\|v_0}$.

%     Let us assume that some player $i$ has a deviation $\sigma'_i$ from $\bsigma^n$ in $\Game_{\|v_0}$.
%     Since $\bsigma^n$ is memoryless, we can assume that $\sigma'_i$ is positional by TODO.
%     and since $\bsigma^n$ is an RSE in the game $\Game^n$, the strategy $\sigma'_i$ uses an edge that does not belong to $E_n$, i.e. there exists $v$ accessible from $v_0$ in $(V, E_n)$ and $vw \in E \setminus E_n$ such that $w = \sigma'_i(v)$.
%     Since only edges controlled by pessimists have been removed, we can immediately deduce that player $i$ is a pessimist.
    
%     Now, among such edges, we choose one whose removal is the most ancient, i.e. we choose it in order to minimize the index $k$ such that $vw \in E_k \setminus E_{k+1}$.
%     Thus, in the strategy profile $(\bsigma^n_{-i}, \sigma'_i)$, it is almost sure that only edges of $E_k$ are used.

%     The fact that the edge $uv$ has been removed at step $k$ means that we had $v \not\in W_k$ and $w \in W_k$.
%     Thus, from the vertex $w$, if player $i$ uses only edges of $E_k$ and the other players follow the strategy profile $\bsigma^k_{-i}$, with positive probability, player $i$ gets the payoff $y_k$ or less.
%     We can already note that the strategy $\sigma'_i$ uses only edges of $E_k$.
%     Moreover, using the reasoning with which we proved that $W_k$ was nonempty, if $y_k \neq 0$ or less is obtained by reaching a terminal $t$, then we have $t \in W_k$ and with positive probability the terminal vertex $t$ is reached without leaving $W_k$.
%     And similarly, if $y_k$ or less is obtained by reaching no terminal, then with positive probability a vertex $u$ is reached without leaving $W_k$, such that from $u$, no terminal is accessible anymore: in both cases, we can say that $w$ is such that if, from $w$, player $i$ uses only edges of $E_k$, and the other players follow the strategy profile $\bsigma^k_{-i}$, then with positive probability player $i$ gets the payoff $y_k$ or less \emph{and} the set $W_k$ is never left.
    
%     Now, the set $E_{k+1}$ was defined so that $W_k$ is no longer accessible from $v_0$ in the graph $(V, E_{k+1})$.
%     Therefore, those vertices are not accessible at any step $\l > k$, and therefore no outgoing edge of a vertex of $W_k$ is ever removed in the sequel, i.e. $E_n \cap (W_k \times V) = E_k \cap (W_k \times V)$.
%     Consequently, since $\sigma'_i$ uses only edges of $E_k$, when the strategy profile $(\bsigma^n, \sigma'_i)$ is played from $w$, it is also true that with positive probability player $i$ gets the payoff $y_k$.
%     And therefore, we have $\X(\bsigma^n_{-i}, \sigma'_i)[\mu_i] \leq y_k$.

%     Let us now prove that $y_k = \X(\bsigma^k)[\mu_i] < \X(\bsigma^n)[\mu_i]$.
%     That is a consequence of the fact that the sequence $(z_\l) = \left(\X(\bsigma^\l)[\mu_i]\right)_\l$ of player $i$'s risk entropies is strictly increasing.
%     Indeed, let us assume $z_{\l+1} \leq z_\l$ for some $\l$.
%     That implies that, in the strategy profile $\bsigma^{\l+1}$, player $i$ has a positive probability of getting the payoff $z_\l$ or less.
%     Then, either there is a positive probability of reaching a terminal vertex that gives them a payoff $z_\l$ or less, or there is a positive probability of reaching no terminal vertex at all.

%     The first case is impossible, because all the terminal vertices that have positive probability of being reached when following $\bsigma^{\l+1}$, i.e. that are accessible from $v_0$ in $(V, E_{\l+1})$, are also accessible from $v_0$ in $(V, E_\l)$, and therefore have positive probability to be reached when following $\bsigma^\l$.

%     In the second case, with the same reasoning as above, there is in particular, a vertex $v$ that has positive probability to be visited infinitely often when $\bsigma^{\l+1}$ is played from $v_0$, and therefore such that if $\bsigma^{\l+1}$ is played from $v$, the probability of reaching a terminal vertex is $0$, i.e. no terminal vertex is accessible from $v$ in $(V, E_{\l+1})$.
%     But then, the vertex $v$ belongs to the set $W_\l$.
%     Indeed, let $j$ be the player that was controlling the edges that were removed at step $\l$.
%     Consider a strategy $\tau_j$ of player $j$ that uses only edges of $E_\l$.
%     Then, when the strategy profile $(\bsigma^\l_{-j}, \tau_j)$ is played, it will almost surely be true that either no terminal vertex is reached, leading to the payoff $0$, or an edge of $E_\l \setminus E_{\l+1}$ is taken, leading therefore to a vertex of $W_\l$, and to a risk entropy of $y_\l$ or less.
%     Thus, since all rewards are non-negative and therefore $y_\l \geq 0$, the vertex $v$ belongs to $W_\l$, which is impossible since it should then have been made inaccessible in the graph $(V, E_k)$.

%     The sequence $(z_\l)_\l$ is therefore strictly increasing, and as a consequence we have $y_k = z_k < \X(\bsigma^n)[\mu_i]$.
%     But then, the deviation $\sigma'_i$ is not a profitable deviation, which is a contradiction.
%     The strategy profile $\bsigma^n$ is a memoryless RSE.

%     \paragraph*{Algorithm}

%     The proof that is given immediately yields an algorithm.
%     Let us comment on its complexity.
%     At each step, at least on edge is removed: we have therefore $\Oh(m)$ such steps.

%     Now, each step starts with checking whether $\bsigma^n$ is an RSE, i.e. by checking, for each player $i$, whether that player $i$ has a profitable deviation.
%     That can be done by computing the set $W_n$ that corresponds to player $i$: player $i$ has a profitable deviation if and only if $v_0 \in W_n$.
%     The computation of the set $W_n$, for a given player $i$, can be done in time $\Oh(m)$ by TODO; and there are $p$ players.
%     Then, the step is finished by removing all the edges leading to $W_n$, which also takes time $\Oh(m)$.

%     Hence the complexity $\Oh(m^2 p)$.
% \end{proof}


==> 6Restrictions.tex <==
% Finally, we consider two further restrictions on the problem to show the tractability border of this problem, and if there are cases where the problem can be solved more efficiently, 
% We show in \cref{thm:infinite_rho_restricted_strategy_np_easy} that restricting the memory or amount of randomness of the strategy still renders the problem $\NP$-complete. 

% Based on observation of the $\NP$-hardness proof requiring only pessimistic players, we show that if instead all the players are optimists, then the problem becomes solvable in polynomial time. 

% \subsection{Restrictions on strategies} 
% First, we consider restrictions on the kinds of strategies used. That is, if the strategy are memoryless, positional or pure. We show that even in such cases finding an RSE is $\NP$-complete. 
% \begin{theorem}\label{thm:infinite_rho_restricted_strategy_np_easy}
%     The constrained existence problem of $(P,O)$-RSEs is $\NP$-complete
%     when the number of players is fixed, even when the players are restricted to positional, memoryless,  or pure strategies. 
% \end{theorem}
% \begin{proof}
%     The lower bound for all three of the above cases follow from \cref{lemma:np_hardness}, with the observation that, in the reduction, if an RSE that satisfies the constraints, then the strategies of the players are positional strategies, and therefore are both pure and memoryless too. 

%     For the upper bound, we show that we can still guess a strategy and verify in polynomial time if it is indeed a strategy. For the cases of positional and memoryless strategies, guessing a strategy is straightforward. Whereas for pure strategies, this requires some work. 
%     \paragraph*{Positional strategies and memoryless strategies} The size of such a strategy $\sigma$ that is an RSE can be represented using polynomially many bits, since one only needs to guess the set of edges from each vertex that are being used with non-zero probability. From \cref{lm:mpd_ptime}, we can then verify if the given $\sigma$ indeed gives a simple quantitative payoff within the constraints, and also if it is indeed an RSE in polynomial time. 

%     \paragraph*{Pure strategies}
%     \thejaswini{Need to write. Maybe proof sketch is enough. }
%     For pure strategies, the strategies might require more memory to represent. We argue therefore that if there is a winning strategy, there is one that requires only 
% \end{proof}

% \subsection{Everyone is optimistic}
% We consider the case where the perceived reward of each player is computed based on the risk-measure $\pexp$ for optimistic players. In this scenario, we show that the problem is $\PTIME$-complete. 
% \begin{theorem}
%     The constrained existence problem of $(P,O)$-RSE is $\PTIME$-complete where all players are optimists, that is, $P=\emptyset$.
% \end{theorem}
% \begin{restatable}{lemma}{ptimeupperbound}
%     The constrained existence problem for $(P,O)$-RSE is in $\PTIME$ if all players are optimists.    
%     The running time of such an algorithm is at most $\Oh()$ where $n$ is the number of vertices in the graph and $p$ is the number of players.\theju{To compute and write here}
%     Moreover, this polynomial time decision algorithm can be modified to output a succinct representation of an RSE satisfying the constraints, when it exists, in $\Oh()$\theju{Copy}.
% \end{restatable}
% \begin{proof}[Proof Sketch.]
    
% \end{proof}

% Finally, we show that the problem is also $\PTIME$-hard even for the case where there are two players. 
% \begin{restatable}{lemma}{ptimelowerbound}\label{lemma:PTIMEHard}
%     The constrained existence problem for two players RSE is $\PTIME$-hard when both players are optimists.
% \end{restatable}
% We show $\PTIME$-hardness for the problem in the case by giving a log-space reduction from the two player zero sum reachability game. Deciding the winner in two player reachability games is $\PTIME$-complete, with hardness proved for the same problem of alternating graph reachability~\cite[Proposition~6]{Imm81}.

==> Old3EntropicRiskMeasure.tex <==
%\thejaswini{I am more-or-less done writing this now. Need to edit maybe}
The entropic risk measure is a measure of the perceived risk which depends on the risk aversion/inclination of the user through the exponential utility function. 

A \emph{risk parameter} of a player is expressed as a real value $\rho\in\Rb$, where a positive value of $\rho$ indicates a risk-averseness of a player and a negative value indicates risk-inclination of a player.

\begin{definition}[Entropic risk measure]
Given a random variable $X$, the entropic risk measure of the variable $X$, is defined as 
$$\re_{\beta,\rho}[X] = -\frac{1}{\rho} \log_\beta \left( \Eb \left[ \beta^{-\rho X}\right] \right).$$
When $X$ is clear from context, we write $\re_\rho$, or even $\re$, for $\re_{\beta,\rho}$.
\end{definition}

% We show that 
\begin{restatable}{theorem}{REisPEOE}\label{thm:RE=PEorOE}
    Let $X$ be any random variable ranging over $\Rb$, and let $\beta > 1$.
    Then:
    \begin{itemize}
        \item The limit risk entropy of $X$ when $\rho$ tends to $0$ exists, and equals the expectation:
        $$\lim_{\rho \to 0} \re_{\beta,\rho} [X] = \Eb[X].$$
        
        \item The limit risk entropy of $X$ when $\rho$ tends to $+\infty$ exists, and equals the pessimistic expectation:
        $$\lim_{\rho \to +\infty} \re_{\beta,\rho} [X] = \pexp[X].$$
        
        \item The limit risk entropy of player $i$ when $\rho$ tends to $-\infty$ exists, and equals the optimistic expectation:
        $$\lim_{\rho \to -\infty} \re_{\beta,\rho} [X] = \oexp[X].$$
    \end{itemize}
\end{restatable}
% \begin{theorem}
    
% \end{theorem}


\begin{definition}[$\beta\brho$-risk-sensitive equilibrium]
    Let $\Game_{\|v_0}$ be a game, and let $\brho \in (\Rb \setminus \{0\})^\Pi$ be a \emph{risk-sensitivity profile}.
    Then, the strategy profile $\bsigma$ is a \emph{$\beta\brho$-risk-sensitive equilibrium}, or \emph{$\beta\brho$-RSE} for short, if and only if for each player $i$, the strategy $\sigma_i$ is $\beta,\rho$-risk-optimal in the MDP $\MDProc(\bsigma_{-i})$.
\end{definition}


Note that for every $\beta, \beta'$ and every $\gamma$, we have $\re_{\beta\gamma} = \re_{\beta'\gamma'}$ where $\gamma' = \gamma \frac{\ln(\beta)}{\ln(\beta')}$.
Therefore, one could fix $\beta$ (for example, to $\beta = e$) and use only $\gamma$ as a parameter without loss of generality, from a semantic perspective; but the choice of $\beta$ can still have an influence on the computabilities and complexities of the problems we will be interested in.



For a given class $\Cc$ of games, we define the following problems:

\begin{definition}[Constrained existence problem for $(P, O)$-equilibria in the class $\Cc$]
    Given a game $\Game_{\|v_0} \in \Cc$, a partition $P, O$ of $\Pi$, and two payoff vectors $\bx, \by \in \Qb^\Pi$, does there exists a $(P, O)$-equilibrium $\bsigma$ in $\Game_{\|v_0}$ such that $x_i \leq \pexp_{\bsigma}[\mu_i] \leq y_i$ for every $i \in P$, and $x_i \leq \oexp_{\bsigma}[\mu_i] \leq y_i$ for every $i \in O$?
\end{definition}

\begin{definition}[Constrained existence problem for risk-sensitive-equilibria in the class $\Cc$]
    Given a game $\Game_{\|v_0} \in \Cc$, a basis $\beta > 1$, a risk-sensitivity vector $\bgamma \in \Qb^\Pi$, and two payoff vectors $\bx, \by \in \Qb^\Pi$, does there exists an RSE $\bsigma$ in $\Game_{\|v_0}$ such that $x_i \leq \re_{\beta\gamma\bsigma}[\mu_i] \leq y_i$ for every $i \in \Pi$?
\end{definition}

\begin{lemma}\label{lemma:RSEtoQSSG}
Given a quantitative simple stochastic game $\Game|_{v_0}$, 
where the risk-parameter $\rho = (\rho_1,\rho_2,\dots,\rho_{|\Pi|})$ is such that $\rho_i\in \Rb$, 
it can be converted into quantitative simple stochastic game $\Game'|_{v_0}$ on the same underlying graph, with set of players, probability function, such that every player has risk parameter $0$, and the terminal rewards for each player is modified  such that any $(\beta,\rho)$-RSE is a Nash equilibria in $\Game'|_{v_0}$
\end{lemma}
\begin{proof}
    Consider the simple stochastic game $\Game|_{v_0} = \tpl{V,E,\Pi,(V_i)_{i\in \Pi},\p ,\mu}$. We will define $\mu'$ such that $\Game'|_{v_0} = \tpl{V,E,\Pi,(V_i)_{i\in \Pi},\p ,\mu'}$ has a Nash equilibrium if and only if $\Game$ has a $(\beta,\gamma)$-RSE.

    For a terminal vertex, we simply define $\mu_i'(v) = -(\beta^{-\rho\mu_i(v)})$. Consider this function $\modifiedreward{\beta}{\rho}\colon x\mapsto -(\beta^{-\rho x})$ as the modified reward function.  This function is similar to the negative utility function defined in the work of Baier et al.,~\cite{BCMP24}, where they replace terminal rewards with the negative value of the above function in order to compute the winner in a two-player zero-sum game with risk-averse players. 
    
    Observe that for any random variable $X$, we have that 
    \begin{equation}\label{inequality:REvsExp}    
    \re_{\beta,\rho}\left[X\right] \geq r\text{ if and only if }\Eb\left[\modifiedreward{\beta}{\rho}(X)\right] \geq -\beta^{-\rho r}\end{equation}
    since $\re_{\beta,\rho}\left[X\right] = \frac{-1}{\rho}\log_\beta\tpl{\Eb[\beta^{-\rho X}]}$.
    
    Therefore, any Nash equilibria in  $\Game'|_{v_0}$ would imply that there is a strategy $\bsigma$ such that, for all players $i\in\Pi$, in the MDP induced by $\sigma_{-i}$,  the strategy  $\sigma_i$ of player $i$ is an optimal strategy. If for some strategy $\tau_i$ of player $i$, if the value in the Markov chain induced by any $\bsigma' = (\sigma_{-i}, \tau_i)$ then consider the probability distribution $\prob_{\bsigma'}$ over plays. Define a random variable $X'$ where the value of the play in $\Game'$ sampled according to the probability distribution $\prob_{\bsigma'}$. 
    Similarly, let the random variable $Y'$ be the value of a play in game $\Game'$ where the play is sampled according to the probability distribution $\prob_{\bsigma}$. Since $\bsigma$ is a Nash equilibrium, we have that  
     $\Eb\left[Y'\right]\geq \Eb\left[X'\right]$.
     Since the payoffs in $\Game'$ is just $\modifiedreward{\beta}{\rho}(\mu_i(v))$, this implies that $\Eb\left[\modifiedreward{\beta}{\rho}(Y)\right]\geq \Eb\left[\modifiedreward{\beta}{\rho}(X)\right]$, where 
     $X$ and $Y$ are random variables where $X$ and $Y$ are both the value of the play in the original game $\Game$, however the plays of $X$ are sampled where the probability distribution is $\prob_{\bsigma}$ and $\prob_{\bsigma'}$, respectively. 
     From the statement (\ref{inequality:REvsExp}), we have     
     \begin{align*}
         \Eb\left[\modifiedreward{\beta}{\rho}(Y)\right]\geq \Eb\left[\modifiedreward{\beta}{\rho}(X)\right]\text{ if and only if }\\\re_{\beta,\rho}[Y'] \geq -\frac{1}{\rho}\log_\beta\tpl{-\Eb\left[\modifiedreward{\beta}{\rho}(X)\right] } = \re_{\beta,\rho}[X']\\
         \text{ if and only if }\re_{\beta,\rho}[Y']\geq \re_{\beta,\rho}[X']
     \end{align*}
      Therefore the strategy  $\bsigma$ is at least as good as (any strategy where one player deviates) $\bsigma'$ for the player $i$ that deviates, when their rewards are the risk-entropy measure. Thus, this makes $\sigma$ an risk-sensitive equilibrium. %\theju{badly written, need to revise. Will do it tomorrow.}
\end{proof}
\begin{theorem}[Existence of RSE]\label{thm:existanceRSE}
    There is always a (pure) $(\beta,\rho)$-RSE over a simple stochastic game. 
\end{theorem}
\begin{proof}
We know from \cref{lemma:RSEtoQSSG} that there is a Nash equilibrium in a modified game if and only if there is an RSE in a given $(\beta,\rho)$-RSE game. Since a pure Nash equilibrium always exists in a stochastic multi-player games~\cite[Theorem 3.10]{Umm10} (A correction of an existing proof~\cite{CMJ04}), our desired result follows.  
\end{proof}
\begin{proposition}\label{proposition:Undecidable}
    The constrained existence problem for RSE where $\brho \in \Qb^{\Pi}$ is undecidable. Further, even when players are restricted to pure strategies, the problem remains undecidable
\end{proposition}
\begin{proof}
         The undecidability of the constrained existence problem follows from the work of Ummels and Wojtczak~\cite[Theorem 4.9]{UW11} where they show the undecidability of the constrained existence problem for Nash equilibria in the setting with 10 or more players. Since Nash equilibria is a specific instance of the setting of RSE iwhere the risk parameters $\brho$ is $0$ for each player, the undecidability of our setting follows. 
\end{proof}

The Square-root sum problem is a decision problem in numerical analysis that asks given a list of $n$ numbers and a value $t$, if the sum of the square root of these numbers is at most $t$.
It is an open problem to determine if $\SQRTSUM$ lies in the polynomial hierarchy.  

% \begin{lemma}\label{lemma:memorylessRSE}
%         The constrained existence problem for RSE when players are restricted to pure strategies for quantitative simple stochastic games is undecidable.
% \end{lemma}
% \begin{proof}
%\end{proof}
\begin{lemma}\label{lemma:memorylessRSE}
        The constrained existence problem for RSE when players are restricted to memoryless (but stochastic) strategies for quantitative simple stochastic games is \begin{itemize}
            \item in $\PSPACE$ if the risk-parameters for each player $\brho$ as well as the base $\beta$ is algebraic; 
            \item decidable---subject to Shanuel's conjecture---if the risk-parameters for each player $\brho$  is algebraic and the base of the exponent is the Euler's constant $\beta=e$.
            \end{itemize}
        The problem is at least $\NP$-hard as well as $\SQRTSUM$-hard.
\end{lemma}
\begin{proof}
     We remark that a lower bound of $\NP$-hardness and $\SQRTSUM$-hardness  follows from the work of Ummels and Wojtczak~\cite[Theorem 4.4,Theorem 4.6]{UW11}. % where they show $\NP$-hardness for the constrained existence problem for Nash equilibria in the setting with only two players. Since Nash equilibria is a specific instance of the setting of RSE, where the risk parameters of each player is $0$, the $\NP$-hardness follows. 
         For the upper bounds, we appeal to results for the existential theory of the reals, the set of all existential first-order sentences that hold in the ordered field of reals $(\Rb,+,\times,0,1,\leq)$. Our results also closely resemble the proof given by Ummels and Wojtczak~\cite[Theorem 4.5]{UW11}, however, we need to do slightly more work to encode the payoff expressed by the entropic risk measure.
         Therefore, if we allow for the base $\beta$ to be equal to the Eular's constant, then we can express the formula using the existential theory of reals with exponents is decidable, subject to Shanuel's conjecture~\cite{MW95}. We don't describe the details, but only remark that Shanuel's conjecture is a well-known conjecture in the field of transcendental number theory~\cite{Lan66}. 
         
         %Further, we need the results in Baier et al.,~\cite{BCMP24} to reason about computational related to checking if a strategy 

    First observe that the it is enough to verify if there is a memoryless Nash equilibrium in the modified game obtained where all the terminal rewards $\mu_i(v)$ are replaced instead with $-\tpl{\beta^{\rho\mu_i(v)}}$. This follows from \cref{lemma:RSEtoQSSG}. 

    Since the players are restricted to strategies that are memoryless, we give a non-deterministic algorithm that uses the solution to sentences in $\exists\Rb$ if the values of $\beta$ and $\rho$s can be expressed in $\Qb$. If $\beta = e$, then we write such existential first order formulas in $\exp\text{-}\exists\Rb$ (The existential theory of reals with an exponentiation). We use solutions to such solutions as a black-box,. For the rational case, since $\exists\Rb$ is contained in $\PSPACE$ and further $\NPSPACE = \PSPACE$, this gives us a $\PSPACE$ algorithm for the case where $\beta$ and $\rho$ are rationals. 
     
     For a game $\Game|_{v_0} = \tpl{V,E,\Pi,(v_i)_{i\in \Pi}, \p,\mu}$, where $\mu$ is a function from a terminal set of nodes $T$ to values in $\Qb$,\theju{terminal nodes def?} and constraints $\Bar{x}$ and $\Bar{y}$ for each of the $n$ players in $\Pi$, let $S$ be the support of the strategy guessed. 

         \subparagraph*{Writing values of terminals efficiently.}
        For each value $t = \mu_i(v)$, which requires $\ell$ bits to encode, we ensure that there is a formula that uses only polynomially many variables in $\ell$ to encode $\modifiedreward{\beta}{\rho}(t) = -\tpl{\beta}^{-\rho t}$. 

        We assume without loss of generality that $\beta$ is a natural number. If $\beta$ is rational instead, and is represented by a value $a/b$, then individually find $a_1  = a^{\rho t}$ and $b_1 = b^{\rho t}$, and just find $b_1/a_1$, which is just written in $\exists\Rb$ by stating that $\exists  t_r \;\exists a_1'\colon a_1'\times a_1  = 1\land t_r = a_1'\times b_1$.
        Now that we assume that $\beta$ is a rational number, we now deal with fixed finite exponentiation with rational values. Similarly, we can assume without loss of generality that $\rho t$ is a natural number. Indeed, any value $r^{a/b} = r^a\times t^{1/b}$ and $t^{1/b}$ can be written as $\exists y \colon y^b = t$.

        It suffices to show therefore that for two values $b,a$, both natural numbers, $b^a$ can be expressed in $\exists\Rb$ succinctly, using only a formula that has length that is not more a poly-log of $b$ or $a$. 
        Let $a = \sum_{i=0}^{\log_2{a}}a_i 2^i$, where $a_i\in\{0,1\}$ 
        The reasoning follows from the observations below. 
        \begin{itemize}
            \item $b^a = \prod_{i=1}^{\log_2{a}}\tpl{b^{a_i}b^{2^i}}$
            \item  $2^i$ can be expressed in a formula with at most $i+1$ many variables
            \item $b^{2^i}$ further requires at most $i$ many variables to express, because let  $b_i$ represent $b^{2^{i}}$, then $b^{2^{i+1}} = b^{2^i}\times b^{2^i}$.
            \item Finally, using a similar trick, $b$ itself can be represented using at most $\log_2{b}$-many variables. 
        \end{itemize}


    Since we can efficiently represent the variables used for the payoffs of the modified game, we now can write an equation assuming that all terminal rewards are available to us constants. We now specify the variables to be used in the first order formula that we will construct to indicate if the constrained existence problem is satisfied. This is done in three parts. Since we have guessed the support, we first ensure that in fact there are variables corresponding to the probability that only take positive values on the edges corresponding to the support set that we guessed.  
    Then, we write equations using variables that compute the values of the induced Markov chain from this strategies. Finally, we also find a the values corresponding to the MDP obtained for each player when playing against the strategies of all other players. Then we compare if the value of the MDP is at least as large as the underlying Markov chain, for each player to ensure that it is indeed an equilibrium. To write all of this in $\exists\Rb$, we introduce the following variables. 
     \begin{itemize}
         \item one variable  $p_{vw}$ for each pair of vertices $vw$, which corresponds to the probabilities corresponding to the strategy;
         \item a variable $r^i_v$ which corresponds to the risk-entropy of player $i$ from vertex $v$ if they followed the strategy defined by the probabilities above; 
         \item a variable $m^i_v$ which corresponds to the value of the value obtained by player $i$ if the game is treated as an MDP against other players.
     \end{itemize}
 
        
     \subparagraph*{Writing FO formula assuming we have access to values for terminals.}
    The following part of the proof is similar to the one found in Ummels and Wojtczak~\cite[Theorem 4.5]{UW11}, but we provide it to suit our setting, for the sake of completeness. 
    First, we have a formula that  $p_{vw}$ indeed describe a strategy. We further ensure that for stochastic vertices, the value $p_vw$ encodes exactly the value dictated by the probability function $\p$ by the stochastic node
    \begin{align*}
    \Phi_S(\Bar{p})\:= \bigwedge_{v,w\in V}p_{vw}\geq 0\land \bigwedge_{v,w\in V}1\leq p_{vw}
    \land \bigwedge_{i\in \Pi}\bigwedge_{v\in V_i} \tpl{\sum_{w\in E(v)}\p_{vw}=1}\land \\
    \bigwedge_{v\in V_?}p_{vw} =  \p(vw)\land \bigwedge_{vw\in S}p_{vw}> 0 
    \end{align*}
    For a fixed support $S$ of a strategy $\alpha$, it is possible to compute the terminals $T_S$ that have non-zero probability of being reached in the underlying Markov chain that is formed, and the vertices $V_S$ from which such terminals can be reached with non-zero probability. We assign value $\mu_i'(v)$ as the reward for the terminal vertices for player $i$, and the reward $1$ for all vertices that cannot reach any terminal with positive probability ($\modifiedreward{\beta}{\rho}(0) = 1$).
    \[\Omega_S^i(\Bar{p},\Bar{r^i})\:= \bigwedge_{v\in T_S} r^i =\mu_i'(v) \land
                 \bigwedge_{v\notin V_S} r^i_v = 1 \land
                 \bigwedge_{v\in V_S\setminus T_S} \tpl{z^i_w = \sum_{w\in E(v)}\tpl{ p_{vw} r^i_v}}
                 \]     
    Finally, for computing the values of the MDP, we construct a similar FO statement
    \[\Gamma_S^i(\Bar{p},\Bar{m^i}) \:= \bigwedge_{v\in T} m^i =\mu_i'(v) \land
                 \bigwedge_{v\in V_i\\w\in E(v)} m_v^i\geq m_w^i \land
                 \bigwedge_{v\notin V\setminus V_i} \tpl{m^i_w = \sum_{w\in E(v)}\tpl{ p_{vw} m^i_v}}\]
Finally our statement would be $$\exists \Bar{p}\:\exists\Bar{r}\:\exists\Bar{m}\colon \Phi(\Bar{p})\land \bigwedge_{i\in\Pi}\left(\tpl{x^i_{v_0}\leq r^i_{v_0}}\land \tpl{r^i_{v_0}\leq y^i_{v_0}}\land\Omega_S^i(\Bar{p},\Bar{r^i})\land \Gamma_S^i(\Bar{p},\Bar{m^i})\land m_{v_0}^i\leq r_{v_0}^i \right)$$
For rewards that are represented by algebraic numbers that also can be expressed succinctly via $\exists\Rb$, we observe that our above reduction extends naturally. 

\end{proof}\theju{to check if this doesn't hit really low values. Need to bound it}


\begin{lemma}\label{lemma:positionalRSE}
        The constrained existence problem for RSE when players are restricted to pure and positional strategies for quantitative simple stochastic games is  in $\PSPACE$ if the risk-parameters for each player $\brho$ as well as the base $\beta$ is algebraic. Further, the problem is $\NP$-hard.% as well as $\SQRTSUM$-hard.
\end{lemma}
\begin{proof}
    For the lower bounds, we just remark that the corresponding problem of constrained existence of Nash equilibria, when players are restricted to positional strategies is both $\NP$-hard~\cite[Theorem 4.4]{UW11}
    from the work of Ummels and Wojtczak. Since Nash equilibria is a specific instance of the setting of RSE, where the risk parameters of each player is $0$, the $\NP$-hardness for the more general case of RSE follows.
    For the upper bound, we simply observe that the same proof as the one for the upper bound of~\cref{lemma:memorylessRSE} can be adapted to this situation. 
\end{proof}
\section{Computing equilibria for values of risk}

From this point, we will therefore extend, by continuity the definition of $\RE_{\beta,\rho}$ for $\rho = 0$.


\begin{lemma}
    If $\rho \leq \rho'$, then $\re_{\beta,\rho} \geq \re_{\beta \rho'}$.
\end{lemma}

\begin{proof}
    This result was proved in a text book on risk theory~\cite{KGD08} in a slightly different context.

    Let $\rho, \rho' \in \Rb \setminus \{0\}$.
    Let us assume $0 < \rho < \rho'$.
    Then, the mapping $x \mapsto x^{\frac{\rho}{\rho'}}$ is concave, hence by Jensen's inequality we can write:
    $$\Eb\left[ \left(\beta^{-\rho'X}\right)^{\frac{\rho}{\rho'}} \right] \leq \left( \Eb\left[ \beta^{-\rho X} \right] \right)^{\frac{\rho}{\rho'}}.$$
    Then, by applying the mapping $-\frac{1}{\rho} \log_\beta$, we obtain:
    $$-\frac{1}{\rho} \log_\beta \Eb\left[ \left(\beta^{-\rho X}\right) \right] \geq -\frac{1}{\rho} \frac{\rho}{\rho'} \log_\beta \Eb\left[ \beta^{-\rho X} \right],$$
    i.e. $\re_\rho[X] \geq \re_{\rho'}[X]$.

    The case where $\rho$ and $\rho$ are negative is analogous, and the result can be generalized to $\Rb$ using the continuity in $0$.
\end{proof}

In an MDP $\MDProc$, a strategy $\sigma$ is \emph{$\beta,\rho$-risk-optimal} if and only if for every strategy $\sigma'$, we have $\Eb_{\sigma'}[\mu] \leq \Eb_\sigma[\mu]$.


\begin{definition}[Risk-sensitive Equilibria]
    Let $\Game_{\|v_0}$ be a game, and let $\brho \in (\Rb \setminus \{0\})^\Pi$ be a \emph{risk-sensitivity profile}.
    Then, the strategy profile $\bsigma$ is a \emph{$\beta\brho$-risk-sensitive equilibrium}, or \emph{$\beta\brho$-RSE} for short, if and only if for each player $i$, the strategy $\sigma_i$ is $\beta,\rho$-risk-optimal in the MDP $\MDProc(\bsigma_{-i})$.
\end{definition}

==> PCompleteness.tex <==
% \begin{theorem}
%     The constrained existence problem of $\Bar{\rho}$-RSEs in $\PTIME$-complete if all the players are optimists, i.e, $\brho = \tpl{-\infty}^{\Pi}$.
% \end{theorem}

% \subsection{Upper bound}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \thejaswini{working on this}
    \begin{itemize}
        \item \emph{Definition of the algorithm}

  

        The algorithm will proceed by constructing a decreasing sequence $E_0, E_1, \dots$ of subsets of $E$.
        At each step, we will always leave at least one outgoing edge from each vertex, and we will never remove outgoing edges of stochastic vertices.
        In the cycle-averse case, we will keep the induction hypothesis that for each $k \geq 1$, there is never a vertex $v$ that is accessible from $v_0$ in $(V, E_k)$ and such that no terminal vertex is accessible from $v$.
        
        Moreover, a preprocessing computes for each vertex $v$ the adversarial optimistic risk measure the player who controls the vertex $v$ can ensure against every strategy profile from $v$. That is, we compute $\val(v) = \inf_{\btau_{-i}} \sup_{\tau_i} \oexp^\btau)[\mu_i]$ where player $i$ controls $v$. 
        All those values can be computed in time $O(pn)$ by TODO.

        Let $E_0 = E$.
        Step $k$ starts when $E_k$ is defined.

        At each step, we then define the strategy profile $\bsigma^k$ as follows:
        \begin{itemize}
            \item In the cycle-averse case: from each vertex $v$, the strategy profile randomizes uniformly between all the edges $vw \in E_k$.
            Note that, when $k \geq 1$, the induction hypothesis implies that from every vertex $v$ accessible from $v_0$, when following $\bsigma^n$, there is a positive probability $q$, independent of the past history, to reach some terminal vertex, and therefore that the probability of visiting $v$ infinitely often is $\lim_\l (1-q)^\l = 0$.
            Consequently, when the strategy $\bsigma^k$ is followed from $v_0$, it is almost sure that some terminal vertex will eventually be reached.
            
            \item In the cycle-friendly case: from each vertex $v$, when $v$ is seen for the first time, the strategy profile randomizes uniformly between all the edges $vw \in E_k$, and then, when $v$ is visited again, it always replicates the same choice.
            Equivalently, each player initially chooses, at random, a positional strategy, and then follows it\footnote{More generally, our model of randomness can be interpreted by considering that the outcome of each randomized action is simply \emph{revealed} when that action is made, but was already decided (randomly) in the past.
            That approach will often be convenient for those strategy profiles $\bsigma^k$.
            But, in the general case, it should be avoided because it might be counter-intuitive: even if our model allows to consider that the outcome of a randomized action has been decided beforehand, it does not allow the players to \emph{communicate} it beforehand to anyone else.
            But in many cases, they might have an incentive to communicate them: it is therefore more intuitive to consider that those choices are made when they are revealed.}.
            \item  In both cases, if some player $i$ deviates and takes an edge that they are not supposed to take (be it an edge that does not belong to $E_k$ or, in the cycle-friendly case, an edge whose origin has already been seen in the past, and from which a different choice has been made), then all the players switch to the positional strategy profile $\btau^{\dag i}$, where $\btau^{\dag i}_{-i}$ is a positional strategy profile that minimizes the quantity $\sup_{\tau_i} \X({\btau^{\dag i}_{-i}, \tau_i})[\mu_i]$, and $\tau^{\dag i}_i$ is some positional strategy.
        \end{itemize}
       
                
        At step $0$, we define $V_{\frownie}^0$ as the set of terminals that give to some player $i$ a payoff greater than $y_i$, and compute it in time $O(n)$.
        At step $k \geq 1$, we define $V_\bad^k$ as follows: first, we compute the perceived reward $z^k_i$ of each player $i$ in $\bsigma^k$, which can be done in time $O(n^2)$, by computing the set of terminal vertices that are reached with nonzero probability, i.e., that are accessible from $v_0$ in $(V, E_k)$, and by deciding whether there exists a positive probability of reaching no terminal---that is the case if and only if we are in the cycle-friendly case (using the induction hypothesis, since we are at step $k \geq 1$), and there exists a positional strategy profile that uses only vertices of $E_k$ such that there is a positive probability of reaching no terminal.
        Then, the set $V_\bad^k$ is the set of vertices $v$ such that there exists a player $i$ and a vertex $v$ such that $\val(v) > z^k_i$.
        
        In both cases, we compute the set $\Attr(V_{\frownie}^k, E_k)$ in time $O(n+m)$.
        If $v_0 \in \Attr(V_{\frownie}^k, E_k)$, we stop there and answer $\No$.
        Otherwise, we define $F_k$ as being the set $E_k$ in which we have removed every edge $uv$ with $u \not\in \Attr(V_\bad^k, E_k)$ and $v \in \Attr(V_{\frownie}^k, E_k)$ (\emph{first removal} of step $k$).
        Note that every stochastic vertex still has all of its outgoing edges in $F_k$, since if it had an outgoing edge leading to a vertex of $\Attr(V_\bad^k, E_k)$, it would itself belong to $\Attr(V_\bad^k, E_k)$; and that every non-stochastic vertex still has at least one outgoing edge in $F_k$, since if it had all of its outgoing edges leading to a vertex of $\Attr(V_\bad^k, E_k)$, it would itself belong to $\Attr(V_\bad^k, E_k)$.
        
        If we are in the cycle-friendly case, we define $E_{k+1} = F_k$.
        If we are in the cycle-averse case, we compute the set $W_\bad^k$ of vertices $v$ from which there is a positive probability of reaching no terminal, following any strategy profile $\btau$ that uses only edges of $F_k$.\theju{Isn't this $\Attr$ in graph with edges in $F_k$?}\leon{It's the same idea, but then it's the attractor of nothing, like an anti-attractor.} This can be computed in time $O(n+m)$. 
        Then, again, if $v_0 \in W_\bad^k$, we stop there and answer $\No$.
        Otherwise, we define $E_{k+1}$ as the set $F_k$ in which we have removed every edge $uv$ with $u \not\in W_{\frownie^k}$ and $v \in W_{\frownie}^k$ (\emph{second removal} of step $k$).
        With the same argument as above, every stochastic vertex still has all of its outgoing edges, and every non-stochastic vertex still has at least one.
        The invariant is then satisfied: for every vertex $v$ from which no terminal vertex is accessible in $(V, E_{k+1})$, we can construct a strategy profile that guarantees positive probability of reaching no terminal vertex from $v$ by using only edges of $F_k$, and deduce $v \in W_\bad^k$: that vertex is therefore no longer accessible from $v_0$ in $(V, E_{k+1})$.
        
        If $k \geq 1$ and if no edge has been removed during the whole step $k$, then we stop the algorithm there, and answer $\Yes$ if $z^k_i \geq x_i$ for each $i$, and $\No$ otherwise.
        Since the sequence $E_0, E_1, \dots$ is strictly decreasing (except at the last, and possibly the first, steps), the algorithm terminates and takes at most time $O(n^4)$.

        If the algorithm answers $\Yes$ at step $k$, its functional version, in the cycle-friendly case, outputs the set $E_{k+1} = E_k$ as a succinct representation of the strategy profile $\bsigma^{k+1} = \bsigma^k$.
        In the cycle-averse case, it defines the set $E_{k+1}$ (which might be equal to $E_k$) from $E_k$ by removing, one by one, edges $uv$ such that, in the current graph:
        \begin{itemize}
            \item the vertex $u$ is not stochastic and has several outgoing edges;
            \item all the terminal vertices accessible from $v$ are also accessible from $v_0$ without using $uv$;
            \item at least one terminal vertex is accessible from $u$ without using $uv$;
        \end{itemize}
        until there is no such edge.
        This optional step can be done in time $O(n^4)$, and therefore does not increase the complexity given above: we call it the \emph{finishing touches step}.
        Note that the set $E_{k+1}$ still satisfies the induction hypothesis, since no edge $uv$ is ever removed if it leaves no terminal vertex accessible from $u$.
        
        Then, the algorithm outputs the set $E_{k+1}$, as a succinct representation of $\bsigma^{k+1}$.
        

        \item \emph{This algorithm recognizes only positive instances and outputs the representation of an RSE.}

        Let us assume that the algorithm answers $\Yes$ at step $k$: let us show that the strategy profile $\bsigma^{k+1}$ is an RSE that satisfies the desired constraints.
        Note that the algorithm does never answer $\Yes$ at step $0$, hence we necessarily have $k \geq 1$.

        \begin{itemize}
            \item \emph{The strategy profile $\bsigma^{k+1}$ satisfies $\X({\bsigma^{k+1}})[\mu_i] \geq x_i$ for each $i$.}

            Indeed, the algorithm answers $\Yes$ at step $k$ only if the strategy profile $\bsigma^k$ satisfies that constraint.
        In the cycle-friendly case, we have $\bsigma^{k+1} = \bsigma^k$, hence the result is immediate.
        
        In the cycle-averse case, the finishing touches step does not affect the risk entropies: the terminal vertices accessible from $v_0$ in $(V, E_k)$ are still accessible in $(V, E_{k+1})$, and by the induction hypothesis, both $\bsigma^k$ and $\bsigma^{k+1}$ are such that some terminal is almost surely eventually reached.

        
            \item \emph{The strategy profile $\bsigma^{k+1}$ satisfies $\X({\bsigma^{k+1}})[\mu_i] \leq y_i$ for each $i$.}
        
        The set $E_1$ has been defined so that the set $\Attr(V_{\frownie}^0, E)$, and therefore the set $V_{\frownie}^0$, is not accessible from $v_0$ in the graph $(V, E_1)$, and therefore in the graph $(V, E_{k+1})$: thus, it is almost sure in $\bsigma^{k+1}$ that no vertex of $V_{\frownie}^0$ will ever be reached.
        Thus, no terminal that gives to some player $i$ a payoff greater than $y_i$ can be reached.
        Moreover, in the cycle-averse case, i.e. when $y_i \geq 0$ for each $i$, by the induction hypothesis, the probability of never reaching a terminal vertex, which would give each player the payoff $0$, is zero.
        
        % Moreover, in the cycle-averse case, it is almost sure that some terminal vertex is reached, because if there was a positive probability to reach no terminal, there would be a vertex $v$ that would be visited infinitely often with positive probability, and therefore from which there exists a strategy profile of the form $\bsigma^{k+1}_{\|hv}$ such that $v$ is almost surely visited infinitely often (otherwise along every play visiting $v$ infinitely often, at each visit of $v$, there would be a positive probability, greater than or equal to some constant $q > 0$ since $\bsigma^k$ is finite-memory, of not visiting $v$ again, which would imply that the probability of visiting $v$ infinitely often when playing that strategy profile is actually smaller than or equal to $\lim_m (1-q)^m = 0$).
        % In other words, no terminal vertex would be accessible from $v$ in $(V, E_{k+1})$; and since no edge is removed during the finishing touches step that would leave a vertex without any terminal vertex accessible from it, it means that it would also have been also the case in the graph $(V, E_k)$.
        % On the other hand, the second removal of step $k-1$ have made unaccessible all the vertices of the set $W_\bad^{k-1}$: we therefore have $v \not\in W_\bad^{k-1}$, which means that there is a strategy profile $\btau$ that, played from $v$, guarantees that a terminal vertex will be reached almost surely.
        % Such a strategy profile must necessarily guarantee that the set $W_\bad^{k-1}$ is never visited, and therefore makes no use of the edge that are removed during the second removal, and uses only edges that still belong to the set $E_k$.
        % But then, that implies that at least one terminal vertex is accessible from $v$ in the graph $(V, E_k)$, which is a contradiction.


            \item \emph{The strategy profile $\bsigma^{k+1}$ is a $\brho$-RSE.}
        
        Let us assume that some player $i$ has a profitable deviation $\sigma'_i$.
        We can assume without loss of generality that $\sigma'_i$ is pure.        
        Let $z' = \X({\bsigma^{k+1}_{-i}, \sigma'_i})[\mu_i]$.
        We first prove that obtaining the payoff $z'$ is impossible by using only edges of $E_{k+1}$.
        Indeed, since in the strategy profile $\bsigma^{k+1}$, player $i$ gets percieved reward $z^k_i < z'$ (we have proved above that the finishing touches do not change the risk entropies), all the terminal vertices that are accessible from $v_0$ in $(V, E_{k+1})$ give player $i$ a reward that is smaller than $z'$.
        Now, if $z' = 0$ and if in $(\bsigma^{k+1}_{-i}, \sigma'_i)$ there is a positive probability of reaching no terminal, then we must distinguish the cycle-friendly and the cycle-averse case.
        In both cases, let us assume toward contradiction that $\sigma'_i$ uses only edges of $E_{k+1}$.
        
        In the cycle-averse case, since $\bsigma^{k+1}$ randomizes between all the edges of $E_{k+1}$ in a memoryless way, we can assume that $\sigma'_i$ is actually positional, and with the same reasoning as above, if there is a positive probability of reaching no terminal vertex in that memoryless strategy profile, it means that there is a vertex $v$ that has positive probability to be reached and from which it is almost sure that no terminal vertex will be reached, and that $v$ will be visited infinitely often.
        But, since all vertices of $W_\bad^{k-1}$ have been made unaccessible during the second removal of step $k-1$, there must be a terminal vertex $t_1$ that is accessible from $v$ in the graph $(V, E_k)$, and therefore in the graph $(V, E_{k+1})$.
        Let then $h = h_0 \dots h_\l$ be a simple path from $v = h_0$ to some terminal $h_\l = t_1$, and let $h_{\leq m}$ be the longest prefix of $h$ that is compatible with $(\bsigma^{k+1}_{-i}, \sigma'_i)$.
        Then, since that path is compatible with the memoryless strategy profile $\bsigma^{k+1}$, the vertex $h_m$ is necessarily controlled by player $i$ and has another outgoing edge $h_mw$, such that from $w$, when following $(\bsigma^{k+1}, \sigma'_i)$, it is almost sure that $v$ will be visited again --- which implies that in particular $v$ is accessible from $w$.
        But then, since there is a terminal vertex (namely $t_1$) that is accessible from $h_m$ without using the edge $h_m w$, the only reason why that edge would not have been removed during the finishing touches step is that there is a vertex $t_2$, accessible from $w$ in $(V, E_{k+1})$, that is not accessible from $v_0$ in $(V, E_{k+1} \setminus \{h_mw\})$.
        By iterating that process, we can create an infinite sequence of different terminal vertices $t_1, t_2, \dots$, which is of course impossible.
        
        In the cycle-friendly case, since $\bsigma^{k+1}$ can be understood as a strategy profile in which each player chooses at random, initially, one positional strategy and then follows it, saying that there is a positive probability of reaching no terminal vertex in $(\bsigma^{k+1}_{-i}, \sigma'_i)$ is equivalent to saying that there is one positional strategy profile $\btau_{-i}$ such that with positive probability, no terminal vertex is reached \emph{and} the strategy profile $\bsigma^k_{-i}$ is following $\btau_{-i}$.
        Then, the strategy $\sigma'_i$ is such that there is a positive probability of reaching no terminal when following $(\btau_{-i}, \sigma'_i)$, and we can actually also assume without loss of generality that $\sigma'_i$ is positional.
        But then, there is also a positive probability that $\sigma^k_i$ actually follows $\sigma'_i$, hence there already is a positive probability to reach no terminal in $\bsigma^k$, hence $z^k_i \geq 0$, which contradicts the inequality $z^k_i < z'$.
        
        Therefore, the strategy $\sigma'_i$ cannot use only the edges of $E_{k+1}$, and the percieved reward $z'$ is actually obtained after having taken an edge $uv \not\in E_k$ (i.e. there exists $hu$ compatible with $\bsigma^k$ such that $\sigma'_i(hu) = v$ and $\prob_{\bsigma^k_{-i\|hu}, \sigma'_{i\|hu}}(\mu_i = z') > 0$, where $u \in V_i$ is accessible from $v_0$ in $(V, E_k)$).
        But, then, after that edge, the strategy profile $\bsigma^k_{-i}$ is actually following the positional strategy profile $\btau^{\dag i}_{-i}$, which prevents player $i$ from increasing the percieved reward to a value larger than $\val(u)$: therefore, we have $z' \leq \val(u)$.
        But, on the other hand, if the algorithm has answered $\Yes$, it means that we had $\val(u) \leq z^k_i$, which contradicts, again, the inequality $z^k_i < z'$.
        The strategy profile $\bsigma^k$ is therefore an RSE, which satisfies the desired constraints.
        \end{itemize}


\item \emph{This algorithm recognizes all positive instances.}

        Let us assume that we have a positive instance, i.e. that there exists an RSE $\bsigma$ with $\bx \leq \X(\bsigma)[\mu] \leq \by$.
        Let us show that the algorithm will never answer $\No$; and therefore, since it is guaranteed to terminate, that it answers $\Yes$.
             
        To do so, we first prove, by induction, that at the beginning of each step $k \geq 0$, every edge that has positive probability to be eventually taken in $\bsigma$ remains in $E_k$, and that $z^k_i \geq \X(\bsigma)[\mu_i]$ for each $i$.
        (Note that if the algorithm gives an answer at step $k$, then there is no step $k+1$, hence that result may not apply to the strategy profile $\bsigma^{k+1}$ which is output when the answer is $\Yes$ --- in other words, the finishing touches step is the only step that might falsify this result.)
        At step $0$, the result is immediate, since $E_0 = E$.

        % For each step $k$, let $uv$ be a vertex that is not accessible from $v_0$ in the graph $(V, E_k)$.
        % Then, it means that every path from $v_0$ to $u$ in $(V, E)$ uses an edge that has been removed during some step $k' < k$, i.e. traverses a vertex that belongs to some set $\Attr(V_\bad^{k'})$ or (in the cycle-averse case) or $W_\bad^{k'}$.
        % But, in the strategy profile $\bsigma$, all those sets have probability $0$ to be visited.

        At step $1$, if the strategy profile $\bsigma$ uses eventually, with positive probability, an edge that does not belong to $E_1$, i.e. goes with positive probability to a vertex $v \in \Attr(V^0_\bad, E_0)$, then with positive probability, a terminal vertex will be reached that gives to some player $i$ a payoff greater than $y_i$, which is impossible.
        
        Now, if $\bsigma$ uses with positive probability an edge that is removed during the first removal of step $k$, then it visits with positive probability a vertex $v \in \Attr(V^k_\bad, E_k)$, and therefore, with positive probability, a vertex $w$ with $\val(w) > z^k_i$, where $i$ is the player controlling $w$.
        But then, in the strategy profile $\bsigma$, player $i$ has a deviation that gives them a percieved reward greater than $z^k_i$.
        Since $\bsigma$ is an RSE, that deviation cannot be profitable, hence we must have $\X(\bsigma)[\mu_i] > z^{k'}_i$.
        Let us show that this is not possible, by showing that every payoff vector that has positive probability to be generated in $\bsigma$ also have positive probability to be generated in $\bsigma^k$.
        By induction hypothesis, all the terminal vertices that are reached with positive probability in $\bsigma$ are also reached with positive probability in $\bsigma^k$.
        If, now, there is a positive probability of getting the zero payoff vector by reaching no terminal in $\bsigma$, it will also be the case in $\bsigma^k$.
        Indeed, if that is the case, we are necessarily in the cycle-friendly case (otherwise $\bsigma$ would not match the constraints given in the instance).
        Then, if $u$ is a vertex that has positive probability to be visited infinitely often in $\bsigma$, then there is a strategy profile (namely $\bsigma$) that uses only vertices that have positive probability to be reached in $\bsigma$, and therefore only edges of $E_k$ by induction hypothesis, that guarantees that with positive probability, the vertex $u$ is visited infinitely often; therefore, there also exists a positional strategy profile giving the same guarantees, and there is a positive probability that $\bsigma^k$ follows that positional strategy profile, hence there is a positive probability of reaching no terminal vertex in $\bsigma^k$.
        This proves that all the payoff vectors that have positive probability to be achieved in $\bsigma$ also have positive probability to be achieved in $\bsigma^k$, and therefore that $\X(\bsigma)[\mu_i] \leq \X({\bsigma^k})[\mu_i] = z^k_i$, which is a contradiction.

        Finally, if we are in the cycle-averse case and there is a positive probability that the strategy profile $\bsigma$ uses an edge that has been removed during the \emph{second} removal of step $k$, and therefore to reach a vertex of $W^k_\bad$: then, since we have already proven that $\bsigma$ uses only edges of the set $F_k$, we deduce that $\bsigma$ is such that with positive probability, no terminal vertex is reached, which is impossible in the cycle-averse case.


        To conclude, the answer $\No$ can be given only in the two following cases:
            \begin{itemize}
                \item \emph{If at step $k$, we have $v_0 \in \Attr(V^k_\bad, E_k)$, or $v_0 \in W_0^k$ in the cycle-averse case.}

                Then, the strategy profile $\bsigma$ visits that set with positive probability, and we have already shown that it was impossible.

                \item \emph{If during step $k$, no edge is removed, but we have $z^k_i < x_i$ for some player $i$.}

                We have shown above that $\X(\bsigma)[\mu_i] \leq \X({\bsigma^k})[\mu_i] = z^k_i$: that case is therefore also impossible by definition of $\bsigma$.
            \end{itemize}

            None of those cases is possible, hence our algorithm will eventually answer $\Yes$.
    \end{itemize} 
\end{proof}

% \begin{proof}
%     \leonard{Old inefficient proof 2}

%     In all this proof, when $W$ is a set of vertices, we write $\Attr(W)$ the \emph{probabilistic attractor} of $W$, i.e. the set of vertices $v$ from which all the players together cannot avoid reaching $W$, i.e. such that following any strategy profile $\bsigma$, there is a positive probability of reaching $W$.
%     By TODO, given $W$, the set $\Attr(W)$ can be computed in time $O(n)$.
    
%     \begin{itemize}
%         \item \emph{Definition of the algorithm}

%         Before starting the algorithm, we need two distinguish two cases: the \emph{cycle-averse} case, in which there exists a player $i$ such that $y_i < 0$ (and therefore in which the requirement $\bx \leq \X(\bsigma)[\mu] \leq \by$ implies that $\bsigma$ must almost surely reach a terminal), and the \emph{cycle-friendly} case, in which there is no such player.
%         The algorithm will work slightly differently in those two cases.

%         The algorithm with proceed by constructing a decreasing sequence $E_0, E_1, \dots$ of subsets of $E$.
%         At each step, we will always leave at least one outgoing edge from each vertex, and we will never remove outgoing edges of stochastic vertices.
%         Moreover, a preprocessing computes for each vertex $v$ the maximal risk entropy $\val(v) = \inf_{\btau_{-i}} \sup_{\tau_i} \X(\btau)[\mu_i]$ that player $i$, the player who controls the vertex $v$ can ensure against every strategy profile from $v$.
%         All those values can be computed in time $O(pn)$ by TODO.

%         Let $E_0 = E$.
%         Step $k$ starts when $E_k$ is defined.
                
%         At step $1$, let $V_{\frownie}^1$ be the set of terminals that give to some player $i$ a payoff greater than $y_i$.
%         In the cycle-averse case, we add to $V_\bad^1$ the set of vertices from which no terminal is accessible in $(V, E)$.
%         Then, we compute the set $\Attr(V_{\frownie}^1)$ in time $O(n)$.
%         If $v_0 \in \Attr(V_{\frownie}^1)$, then we stop the algorithm there and answer $\No$.
%         Otherwise, let us define $E_2$ by removing all the edges that go from a vertex that does not belong to $\Attr(V_{\frownie}^1)$ to a vertex that does.

%         Step $k \geq 2$ start once the set $E_k$ is defined.
%         % We then define the strategy profile $\bsigma^k$ as follows:
%         % \begin{itemize}
%         %     \item in the cycle-averse case: from each vertex $v$, the strategy profile randomizes uniformly between all the edges $vw \in E_k$\footnote{Actually, we could have defined $\bsigma^k$ in the cycle-averse case in the same fashion as in the cycle-friendly case, since edges have been removed at step $1$ to avoid cycling where that was possible.
%         %     But this distinction enables us to have a memoryless strategy profile, and it will therefore enable us to show that, in the cycle-averse case, if an };
%         %     \item in the cycle-friendly case: from each vertex $v$, when $v$ is seen for the first time, the strategy profile randomizes uniformly between all the edges $vw \in E_k$, and then, when $v$ is visited again, it always replicates the same choice.
%         %     Equivalently, each player initially chooses, at random, a positional strategy, and then follows it\footnote{The different positional strategies may not have the same probability to be followed, but they all have a positive probability.
%         %     A rigorous proof of the equivalence can be infered from TODO.
%         %     We will however avoid that approach here, since assuming that the players choose from the start which positional strategy they are going to follow could easily lead to believe that they can communicate that choice between them, so that the players can act differently depending on what the other players plan to do in the future.
%         %     But, in our model, each player's actions can depend only on the actual history that has been realized.}.
%         % \end{itemize}
%         % In both cases, if a player $i$ deviates and takes an edge that they are not supposed to take (be it an edge that does not belong to $E_k$ or, in the cycle-friendly case, an edge whose origin has already been seen in the past, and from which a different choice has been made), then all the players switch to the positional strategy profile $\btau^{\dag i}$, where $\btau^{\dag i}_{-i}$ is a positional strategy profile that minimizes the quantity $\sup_{\tau_i} \X({\btau^{\dag i}_{-i}, \tau_i})[\mu_i]$, and $\tau^{\dag i}_i$ is some positional strategy.
%         We then define the strategy profile $\bsigma^k$ as follows: from each vertex $v$, when $v$ is seen for the first time, the strategy profile randomizes uniformly between all the edges $vw \in E_k$, and then, when $v$ is visited again, it always replicates the same choice.
%         Equivalently, each player initially chooses, at random, a positional strategy, and then follows it\footnote{The different positional strategies may not have the same probability to be followed, but they all have a positive probability.
%         A rigorous proof of the equivalence can be infered from TODO.
%         We will however avoid that approach here, since assuming that the players choose from the start which positional strategy they are going to follow could easily lead to believe that they can communicate that choice between them, so that the players can act differently depending on what the other players plan to do in the future.
%         But, in our model, each player's actions can depend only on the actual history that has been realized.}.        
%         If a player $i$ deviates and takes an edge that they are not supposed to take (be it an edge that does not belong to $E_k$, or an edge whose origin has already been seen in the past, and from which a different choice has been made), then all the players switch to the positional strategy profile $\btau^{\dag i}$, where $\btau^{\dag i}_{-i}$ is a positional strategy profile that minimizes the quantity $\sup_{\tau_i} \X({\btau^{\dag i}_{-i}, \tau_i})[\mu_i]$, and $\tau^{\dag i}_i$ is some positional strategy.

%         Computing the risk entropy $z^k_i$ of each player $i$ in $\bsigma^k$ can be done in time $O(n)$, by computing the set of terminal vertices that are reached with nonzero probability, i.e. that are accessible from $v_0$ in $(V, E_k)$, and by deciding whether there exists a positive probability of reaching no terminal --- which is the case if and only if there exists a positional strategy profile that uses only vertices of $E_k$ such that there is a positive probability of reaching no terminal.
%         Then, we can also check in time $O(n)$ whether there exists a player $i$ and a vertex $v$ such that $\val(v) > z_i$.
%         If that is not the case, then we stop the algorithm there, and answer $\Yes$ if $z^k_i \geq x_i$ for each $i$, and $\No$ otherwise.
%         Otherwise, we compute in time $O(n)$ the set $V_{\frownie}^k = \{v \in V_i ~|~ \val(v) > z^k_i\} \neq \emptyset$, and the set $\Attr(V_{\frownie}^k$.
%         If $v_0 \in \Attr(V_{\frownie}^k)$, we stop there and answer $\No$.
%         Otherwise, we define $E_{k+1}$ as the set $E_k$ in which we have removed every edge $uv$ with $u \not\in V_{\frownie^k}$ and $v \in V_{\frownie}^k$.

%         The algorithm does necessarily terminate, since the sequence $E_0, E_1, \dots$ is strictly decreasing.


%         \item \emph{This algorithm recognizes only positive instances.}

%         If the algorithm answers $\Yes$ at step $k$, then the strategy profile $\bsigma^k$ satisfies $\X({\bsigma^k})[\mu_i] \geq x_i$ for each $i$.
%         Moreover, we necessarily have $k \geq 2$, and the set $E_2$ has been defined so that the set $\Attr(V_{\frownie}^1)$, and therefore the set $V_{\frownie}^1$, is not accessible from $v_0$ in the graph $(V, E_2)$, and therefore in the graph $(V, E_k)$: therefore, it is almost sure in $\bsigma^k$ that no vertex of $V_{\frownie}^1$ will be reached.
%         Thus, no terminal that gives to some player $i$ a payoff greater than $y_i$ can be reached.
%         Moreover, in the cycle-averse case, it is almost sure that some terminal vertex is reached, because if there was a positive probability to reach no terminal, there would be a vertex $v$ that would be visited infinitely often with positive probability, and therefore from which there exists a strategy profile of the form $\bsigma^k_{\|hv}$ such that $v$ is almost surely visited infinitely often (otherwise along every play visiting $v$ infinitely often, at each visit of $v$, there would be a positive probability, greater than or equal to some constant $q > 0$ since $\bsigma^k$ is finite-memory, of not visiting $v$ again, which would imply that the probability of visiting $v$ infinitely often is actually smaller than or equal to $\lim_m (1-q)^m = 0$).
%         But then, by the property of $E_1$ in the cycle-averse case that we have proven when constructing $E_1$, the vertex $v$ is such that no terminal is accessible from $v$ in $(V, E)$, and therefore that $v \in V_\bad^1$, which is a contradiction.        
%         Thus, it is almost sure, when following $\bsigma^k$, that no player $i$ will get a payoff greater than $y_i$.
%         Consequently, we also have $\X({\bsigma^k})[\mu_i] \leq y_i$ for each $i$.
        
%         Finally, let us assume that some player $i$ has a profitable deviation $\sigma'_i$.
%         We assume without loss of generality that $\sigma'_i$ is pure.
%         Let $z' = \X({\bsigma^k_{-i}, \sigma'_i})[\mu_i]$.
%         Obtaining the payoff $z'$ is impossible by using only edges of $E_k$.
%         Indeed, since in the strategy profile $\bsigma^k$, player $i$ gets risk entropy $z^k_i < z'$, all the terminal vertices that are accessible from $v_0$ in $(V, E_k)$ give player $i$ a reward that is smaller than $z'$.
%         Moreover, if $z' = 0$ and if in $(\bsigma^k_{-i}, \sigma'_i)$ there is a positive probability of reaching no terminal, then there is in particular one positional strategy profile $\btau_{-i}$ such that with positive probability, no terminal vertex is reached \emph{and} the strategy profile $\bsigma^k_{-i}$ is following $\btau_{-i}$.
%         Then, the strategy $\sigma'_i$ is such that there is a positive probability of reaching no terminal when following $(\btau_{-i}, \sigma'_i)$, and we can actually assume without loss of generality that $\sigma'_i$ is positional.
%         But then, there is also a positive probability that $\sigma^k_i$ actually follows $\sigma'_i$, and that event is independent of $\bsigma^k_{-i}$, hence there already is positive probability to reach no terminal in $\bsigma^k$, which is a contradiction.
        
%         Therefore, the risk entropy $z'$ is actually obtained after having taken an edge $uv \not\in E_k$ (i.e. there exists $hu$ compatible with $\bsigma^k$ such that $\sigma'_i(hu) = v$ and $\prob_{\bsigma^k_{-i\|hu}, \sigma'_{i\|hu}}(\mu_i = z') > 0$, where $u \in V_i$ is accessible from $v_0$ in $(V, E_k)$).
%         But, then, after that edge, the strategy profile $\bsigma^k_{-i}$ is actually following the positional strategy profile $\btau^{\dag i}_{-i}$, which prevents player $i$ to get a risk entropy better than $\val(u)$: therefore, we have $z' \leq \val(u)$.
%         But, on the other hand, if the algorithm has answered $\Yes$, it means that we had $\val(u) \leq z^k_i$, which, again, contradicts the inequality $z^k_i < z'$.
%         The strategy profile $\bsigma^k$ is therefore an RSE, which satisfies the desired constraints.


%         \item \emph{This algorithm recognizes all positive instances.}

%         Let us assume that we have a positive instance, i.e. that there exists an RSE $\bsigma$ with $\bx \leq \X(\bsigma)[\mu] \leq \by$.
%         Let us prove by induction that for every $k \geq 1$, if a vertex is almost surely never visited in $\bsigma^k$ (i.e. if it is not accessible from $v_0$ in $(V, E_k)$), then it also is in $\bsigma$, and that $z^k_i \geq \X(\bsigma)[\mu_i]$ for each $i$.

%         For $k = 1$, be it in the cycle-friendly or the cycle-averse case, the vertices accessible form $v_0$ in $(V, E_1)$ are the same as in $(V, E)$, since an edge $uv$ is removed only if $u$ is accessible from $v$ and from $v_0$.
        
        
%         Let $uv$ be an edge that is removed at step $k \geq 1$, i.e. such that $uv \in E_k \setminus E_{k+1}$.
%         Then, it is almost sure that the vertex $v$ is never visited in $\bsigma$.
%         Indeed, if the edge $uv$ has been removed at step $k$, then it means that we had $v \in \Attr(V_\bad^k)$.
%         Therefore, if we assume that the strategy profile $\bsigma$ visits $v$ with positive probability, then there is also a positive probability that it visits $V_\bad^k$.
%         If $k = 1$, then from each vertex of $V_\bad^1$, there is a positive probability that some player $i$ gets a payoff that is greater than $y_i$, which is impossible.
%         If now $k \geq 2$, then $V^k_\bad$ was defined as the set of vertices $w$ with $\val(w) > z^k_i$, where $i$ is the player controlling $w$: since the sequence $(z^k_i)_k$ is non-increasing (the set of terminal vertices that are accessible from $v_0$ in $(V, E_\l)$ is non-increasing, and if there is a positive probability to reach no terminal in $\bsigma^{\l+1}$, then it was also the case in $\bsigma^\l$).
%         Thus 
%     \end{itemize}
% \end{proof}







% \begin{proof}
%     \leonard{Old inefficient proof 1}

%     \begin{itemize}
%         \item \emph{Definition of $\bsigma^{Wp}$}

%         Let $p \in [0,1]$, and let $W$ be a stable vertex set in $\Game_{\|v_0}$.
%         Let $v_\circlearrowleft$ be a vertex.
%         We define the finite-memory strategy profile $\bsigma^{Wp}$ as follows:

%         \begin{itemize}\item At first (when reading the vertex $v_0$), each player's memory initializes in the state $\cycle$ if $p=0$, and in the state $\terminals$ otherwise.

%         \item When the players' memories are in the state $\cycle$, the strategy profile $\bsigma$ follows some pure memoryless strategy $\btau_{\circlearrowleft}$ that goes only to vertices that belong to $W$, and such that, if possible, the probability of never reaching a terminal vertex is nonzero.
%         Then, the players' memories stay in the state $\cycle$, unless some player $i$ deviates and uses an edge that they are not supposed to use: then, they switch to the state $\punish_i$. 

%         \item When the players' memories are in the state $\terminals$, if $p = 1$, the strategy profile $\bsigma$ follows the memoryless strategy profile $\btau_{\curlywedgedownarrow}$, which consists in, from every vertex $v \in W$, taking each of the edges $vw \in W \times W$ with some nonzero probability.
%         Note that since $v_0 \in W$, that is always possible until some player $i$ deviates and takes an edge to a vertex $w \not\in W$.
%         Then, the collective memory switches to the state $\punish_i$.

%         \item When the players' memories are in the state $\terminals$, if $p < 1$, the strategy profile $\bsigma$ follows the memoryless strategy profile $\btau_{\curlywedgedownarrow \circlearrowleft}$, which consists in, from every vertex $v \in W$, taking each of the edges $vw \in W \times W$ with some nonzero probability.
%         Then, when the vertex $v_\circlearrowleft$ is visited, all the players switch their memories to the state $\terminals$.
%         When some player $i$ deviates and moves to a vertex that does not belong to $W$, all the players switch their memories to the state $\punish_i$.

%         \item When the players' memories are in the state $\terminals_{v_0}$, they behave exactly as when they are in the state $\terminals$, except for the fact that if the vertex $v_\circlearrowleft$ is visited once again, they switch to the state $\cycle$ (which is therefore reached when the vertex $v_\circlearrowleft$ is visited twice).

%         \item When the players' memories are in the state $\punish_i$ for some player $i$, the strategy profile $\bsigma$ follows some memoryless pure strategy profile $\btau_{\dag_i}$, where $\btau_{\dag_i -i}$ minimizes the risk entropy $\max_{\tau_i} \X({\btau_{\dag_i -i}, \tau_i})[\mu_i]$ that player $i$ can get (such a pure memoryless strategy profile exists by Lemma~\ref{lm:reach_safe_positional}), and where $\sigma_{\dag_i i}$ is chosen arbitrarily.
%     \end{itemize}


%     \item \emph{If there is a $\brho$-RSE $\bsigma$ in $\Game_{\|v_0}$ that satisfies $\bx \leq \X(\bsigma)[\mu] \leq \by$, there is one of the form $\bsigma^{Wp}$.}

%     Let us assume the existence of such $\bsigma$.
%     Let $W$ be the set of vertices that have nonzero probability of being reached in $\bsigma$, and let $p$ be the probability of reaching a terminal vertex when following $\bsigma$.
%     If $p < 1$, i.e. if there is a nonzero probability of reaching no terminal, then we can choose a vertex $v_\circlearrowleft$ that has nonzero probability to be visited infinitely often.
%     Let us show that the corresponding strategy profile $\bsigma^{Wp}$ is also a $\brho$-RSE satisfying the desired constraints.

%     \begin{itemize}
%         \item \emph{It generates the same risk entropies as $\bsigma$.}

%         Indeed, the payoff vectors that have nonzero probability to be obtained in $\bsigma$ and in $\bsigma^{Wp}$ are the same.
%         That result is immediate for payoff vectors that are obtained by reaching a terminal, since the vertices, including the terminal vertices, that have nonzero probability to be reached in $\bsigma^{Wp}$ are exactly the vertices of $W$, i.e. the same as in $\bsigma$.

%         Now, let us show that if there is a nonzero probability of reaching no terminal in $\bsigma$, i.e. if $p < 1$, then that is also the case in $\bsigma^{Wp}$.
%         If $p = 0$, then the collective memory initializes in state $\cycle$, and since there is a strategy profile that avoids terminal vertices with nonzero probability, that is also what the strategy profile $\btau_{\circlearrowleft}$ does, and therefore so does $\bsigma^{Wp}$.
%         If $0 < p < 1$, then $\bsigma^{Wp}$ starts in the memory states $\terminals$.
%         Since the vertex $v_\circlearrowleft$ has nonzero probability to be visited infinitely often in $\bsigma$ there is a path from $v_0$ to $v_\circlearrowleft$, and then from $v_\circlearrowleft$ to itself, that traverses only vertices of $W$.
%         Therefore, with nonzero probability, the strategy profile $\bsigma^{Wp}$ visits twice that vertex and, then, switches to the state $\cycle$.
%         Then, for the same reason as above, with nonzero probability, no terminal is reached.

%         Conversely, if in $\bsigma^{Wp}$, with nonzero probability, no terminal vertex is reached, then it can be because the collective memory has switched to the state $\cycle$, and that is possible only if $p < 1$, or because the subgraph of $(V, E)$ induced by $W$ contains a strongly connected component that is not a terminal vertex without any outgoing edge leading to a vertex in $W$.
%         If that is the case, it means that a given vertex $v$ of that strongly connected component has nonzero probability to be visited in $\bsigma$, but that no terminal vertex can be reached with nonzero probability after $v$ has been visited.
%         In that case too, we have $p < 1$, i.e. in $\bsigma$ there is a nonzero probability that no terminal vertex is reached.


%         \item \emph{No optimist has a profitable deviation.}

%         \leonard{Oops: what about undetectable deviations that cycle?}
%     \end{itemize}
%     \end{itemize}
% \end{proof}



% \subsection{Upper bound}

% \begin{lemma}
%     The constrained existence problem of $\Bar{\rho}$-RSE is in $\PTIME$ if all the players are optimists. 
% \end{lemma}

==> zzoldproofNPEasy.tex <==
\leonard{Just adding some results I am using later}

\begin{lemma} \label{lm:mpd_ptime}
    Given a simple quantitative MDP $\MDProc$, the quantities $\max_\sigma \pexp_\sigma[\mu]$ and $\sup_\sigma \oexp_\sigma[\mu]$ can be computed in polynomial time.
    As a consequence, the pessimistic and optimistic expectation of a simple quantitative payoff function can also be computed in polynomial time in a Markov chain.
\end{lemma}

\begin{proof}
    \leonard{todo}
\end{proof}



\subsection{Examples}

\leonard{Add here some examples to explain the concept of anchoring players.}


\subsection{Lower bound}


%    \leonard{Thejaswini, this is for you.}
\input{5NPhardness}



\subsection{Upper bound in the general case}
We first prove a small combinatorial lemma that helps bound our memory. 
\input{5NPComplete-Combinatorial}






\begin{lemma}\label{lm:reach_safe_positional}
    Let $\Game$ be a game.
    Let $W$ be a set of vertices, and let $X, Y \subseteq \Rb^\Pi$ be two sets of payoff vectors with $X \cap Y = \emptyset$.
    Then, there exists a positional strategy profile $\bsigma$ such that:
    \begin{itemize}
        \item the elements of $W$ are visited with probability $0$;
        \item some payoff vector of $X$ is achieved with nonzero probability;
        \item the payoff vectors of $Y$ are achieved with probability zero;
    \end{itemize}
    when $\bsigma$ is followed, from any vertex from which some strategy satisfying those constraints exists.
\end{lemma}

\begin{proof}
    Let us define dynamically the edges that must never be taken, and those that can.
    At first, let us assume that all edges are marked as white.
    Let $W'$ be the set of vertices from which, for every chosen strategy profile, some element of $W$ has nonzero probability to be visited, or some payoff vector of $Y$ has nonzero probability to be achieved (in particular, we have $W \subseteq W'$).
    Then, mark as red all the edges $uv$ with $u \not\in W'$ and $v \in W$.
    Note that any $u \not\in W$ has, still, one outgoing edge that remains white, and all outgoing edges that remains white if it is a stochastic node.

    Then, the game $\Game$ without the red edges can be seen as an MDP, where the objective is to reach one of the terminals associated to a payoff vector belonging to $X$ (if $\bar{0} \not\in X$) or to avoid the terminals associated to a payoff that does not belong to $X$ (if $\bar{0} \in X$).
    It is, then, a reachability or a safety objective, for which, by TODO, there exists a positional uniformly optimal strategy (profile) $\bsigma$, which can also be interpreted as a strategy profile in the game $\Game$ (which never takes the red edges), which satisfies our requirements.
\end{proof}

\begin{lemma} \label{lm:rse_finite_memory}
    Let $\Game_{\|v_0}$ be a game with $n$ vertices and $p$ players.
    Let $\bsigma$ be a $\brho$-RSE in $\Game_{\|v_0}$.
    Then, there exists a $\brho$-RSE $\bsigma^\star$ in $\Game_{\|v_0}$ such that $\re_{\bsigma^\star}[\mu] = \re_{\bsigma}[\mu]$ and that has at most $4np -2n + p + 1$ memory states.
\end{lemma}

\begin{proof}
    \leonard{I think I'm done with this proof, but maybe another brain should check it}

    Let $\bsigma$ be a $\brho$-RSE in $\Game_{\|v_0}$.
    Let $\bz = \re_\bsigma[\mu]$.
    Let us first define, for each history compatible with $\bsigma$, which players are currently being anchored.
    From that labelling, we will be able to define a strategy profile $\bsigma^\star$.
    Finally, we will prove that $\bsigma^\star$ is a $\brho$-RSE with $\re_\bsigma[\mu] = \re_{\bsigma^\star}[\mu]$.

\paragraph*{Definition of the labelling $\Lambda$}
    \begin{proposition}[A finite abstraction $\Lambda$ of a strategy]
        There is a labelling $\Lambda: \Comp(\bsigma) \to 2^\Pi$ such that for every history $hv$, where $h\in V^*$, and $v\in V$, and for every player $i\in \Lambda(hv)$ \theju{Check if compliant players are defined before}
        \begin{enumerate}
        \item $\Lambda(h) = \bigcup_{v \in \Supp (\bsigma(h))} \Lambda(hv)$;~\label{itm:partitionanchor}
        \item if $i$ is an optimist, then  $\re_{\bsigma_{\|hv}}[\mu_i] = z_i$;~\label{itm:optimistanchor}

        \item if $i$ is a pessimist, then for every strategy $\tau_i$ for player $i$, we have $\re_{(\bsigma_{-i\|hv}, \tau_i)}[\mu_i] \leq z_i$.~\label{itm:pessimistanchor}
    \end{enumerate}
    \end{proposition}
    \begin{claimproof}
        We define inductively a labelling based on the length of histories $\Lambda: \Comp(\bsigma) \to 2^\Pi$ that satisfies the conditions from the proposition. 
    % , with the following induction hypothesis, for every history $hv$ and for every player $i \in \Lambda(hv)$:
    % \begin{itemize}
    %     \item if $i$ is an optimist, then we have $\re_{\bsigma_{\|hv}}[\mu_i] = z_i$;

    %     \item if $i$ is a pessimist, then for every strategy $\tau_i$, we have $\re_{(\bsigma_{-i\|hv}, \tau_i)}[\mu_i] \leq z_i$.
    %     \item $\Lambda(h) = \bigcup_{v \in \Supp (\bsigma(h))} \Lambda(hv)$.
    % \end{itemize}
    
    First, we define $\Lambda$ for the trivial history $v_0$, the value $\Lambda(v_0) = \Pi$, that is, all players must be anchored.
    Let us notice that the history $v_0$ satisfies the induction hypothesis, which simply states that the pessimists have no profitable deviation, and that the optimists get the optimistic expectation they are supposed to get.
    
    Suppose $\Lambda(hv)$ has already been defined, where $hv$ is a history compatible with $\bsigma$. 
    Let $w_1, \dots, w_k$ be the successors of $v$ that are chosen by the strategy $\bsigma(hv)$ with non-zero probability, that is, the support of $\bsigma(hv)$.
    If $k=1$, then $\Lambda(hvw_1) = \Lambda(hv)$. 
    If not, and $k>1$, we define each $\Lambda(hvw_\l)$  by first declaring it to be the empty set and successively adding vertices from $\Lambda(hv)$ to $\Lambda(hvw_\l)$.
    \begin{claim}\label{claim:successorAnchor}
    If $i \in \Lambda(hv)$ is a pessimistic player who does not control $v$, then   there is a successor $w_\ell$ of $v$, chosen with non-zero probability by $\sigma$ such that for every  strategy $\tau_i^\ell$, we have $\re_{(\bsigma_{-i\|hvw_\ell}, \tau_i)}[\mu_i] \leq z_i$.     
    Instead if $i$ is an optimist, and $\re_{\bsigma_{\|hv}}[\mu_i] = z_i$, then  there is at least one successor $w_\l$ such that $\re_{\bsigma_{\|hvw_\l}}[\mu_i] = z_i$.
    \end{claim}
    \begin{claimproof}
            We prove the above claim using contradiction for pessimists. Suppose not, and for each $w_\l$, there exists a strategy $\tau_i^\l$ such that $\re_{\bsigma_{-i\|hvw_\l}, \tau^\l_i}[\mu_i] > z_i$. Then, the strategy $\tau_i$ defined by $\tau_i(w_\l h') = \tau^\l(h')$ for each $\l$ is such that $\re_{\bsigma_{-i\|hv}, \tau_j}[\mu_i] > z_i$, which is impossible since $\Lambda(hv)$ satisfies the conditions in the proposition.\theju{Contradiction is not necessary here. We can instead prove it directly, from definition.}

            It follows from the definition of $\re$ for an optimistic player. \theju{Is this enough?}
    \end{claimproof}
    \subparagraph*{Vertex $v$ is controlled by a pessimistic player.}
    If the vertex $v$ is controlled by some pessimistic player $i$ who is already anchored at history $hv$, that is, $i \in \Lambda(hv)$, then we add $i$ to  $\Lambda(hvw_\l)$ for all $\ell\in[k]$.
    
    However, if $i \in \Lambda(hv)$ is a pessimistic player who does not control $v$, then from \cref{claim:successorAnchor} that there is a successor $w_\ell$ of $v$  such that for every  strategy $\tau_i^\ell$, we have $\re_{(\bsigma_{-i\|hvw_\ell}, \tau_i)}[\mu_i] \leq z_i$.     
    We pick one such vertex $w_\ell$, and add $i$ to the set $\Lambda(hvw_\l)$.

    Therefore, there exists at least one $w_\l$ such that $\re_{\bsigma_{-i\|hvw_\l}, \tau_i}[\mu_i] \leq z_i$ for all $\tau_i$. 
    Note that this satisfies the Condition~\ref{itm:pessimistanchor}, the induction hypothesis is satisfied.
    \subparagraph*{Vertex $v$ is controlled by an optimistic player.}Now, let us consider an optimistic player $i \in \Lambda(hv)$.
    By the inductive construction of $\Lambda$, we have $\re_{\bsigma_{\|hv}}[\mu_i] = z_i$. 
    Therefore, from \cref{claim:successorAnchor}, there is at least one successor $w_\l$ such that $\re_{\bsigma_{\|hvw_\l}}[\mu_i] = z_i$.
    We then add player $i$ to the set $\Lambda(hvw_\l)$. Note that adding such an $i$ to $\Lambda(hvw_\l)$ ensures Condition~\ref{itm:optimistanchor} is satisfied.

    In both of the above cases for player $i$ being optimistic or pessimistic, if there is more than one $w_\l$ that satisfies the condition in \cref{claim:successorAnchor}, then we chose a $w_\l$ such that the set $\Lambda(hvw_\l)$ is empty.
    
    This way, for all $i \in \Lambda(hv)$, we ensure that we define $\Lambda(hvw_\l)$ that satisfying the three conditions in the proposition for histories $hvw_\ell$.
    \end{claimproof}

\paragraph*{Definition and counting of the memory states}
\thejaswini{Defining and counting needs to be separated. It is too much information at the same time. Counting can be postponed to the end.}
    We define the memory states for a strategy $\bsigma^\star$ that we construct as follows
    \begin{itemize}    
        \item for each player $i$, the state $\punish_i$;

        \item for each vertex $v$ and each subset $P \subseteq \Pi$ of players such that there exists $h$ with $P = \Lambda(h)$, the state $\anchor_{Pv}$;

        \item the state $\anchor_{\Pi\bot}$
    \end{itemize}

    Let us now bound the number of such states.
    There are, obviously, exactly $p$ states of the form $\punish_i$.
    Let us now prove that there are at most $4np-2n$ states of the form $\anchor_{Pv}$ with $v \in V$.
    
    We say that a subset $P$ of player is $\Lambda(h)$-compatible for a given function $\Lambda$ if there is some history $h'$ such that $P = \lambda(hh')$.
    % We further say that a subset $P$ is $\Lambda(h)$-compatible if $P\subseteq \Lambda(h)$, $P$ is $\Lambda$-compatible, and there is an extension of the history $h$ to $hh'$ such that $P = \Lambda(hh')$.

    Let $f(h)$ be the number of $\Lambda(h)$-compatible subsets.
    Clearly, if $|\Lambda(h)| = m$, then $f(h) \leq 2^m$ because every subset such that $P = \lambda(hh')$ is a subset of $\Lambda(h)$.
We show tighter bounds for $\Lambda(h)$.
    \begin{claim}\label{claim:LambdaCompatible}
         If $|\Lambda(h)| = m > 0$ then the number of $\Lambda(h)$-compatible sets is at most $4m-2$, that is, we have $f(h) \leq 4m-2$.
    \end{claim}
    \begin{claimproof}[Proof of \cref{claim:LambdaCompatible}]
        We construct a (directed acyclic) graph where the states of this graph are exactly $\Lambda$-compatible sets. We later show that the such a DAG is indeed a split-graph for the subset $\Lambda(h)$. From \cref{lemma:counting_subset_dag}, our claim follows since the number of vertices in a split-graph of a set $S$ is at most $4|S|-2$.
    \end{claimproof}

    
    \begin{claimproof}
    We 
    \subparagraph*{Strategy $\bsigma$ extends history $h$ uniquely.}If the strategy $\sigma$ after the history $h$ is has a unique extension in history, that is, the strategy is pure and no confirming play visits a stochastic vertex, then 
    for all $h'$, we have $\Lambda(hh') = \Lambda(h)$. Therefore, only the set $\Lambda(h)$ is $\Lambda(h)$-compatible, and therefore, since $m>2$, 
    in such cases we have $f(h) = 1<3m-3$. 
    that is, in any extension $h'$ of the history $h$, then $\Lambda(hh') = \Lambda(h)$.
%    Therefore, if $\bsigma_{\|h}$ is fully deterministic (pure and no confirming play visits a stochastic vertex), then 

    \subparagraph*{Strategy $\bsigma$ on history $h$ has more than one extension.} If the strategy $\bsigma$ after history $h$ does not have a unique extension, then we say that $\Lambda(h)$ \emph{splits}. That is, $\Lambda(h)$ splits if there is an extension $h'v$ such that $v$ is a stochastic node, or $v$ is controlled player $i$ and strategy $\sigma_i(hh'v)$ is a randomized action.

    Let $h'v$ be the shortest history such that $hh'v$ is compatible with $\bsigma$, and that $\bsigma(hh'v)$ is a randomised action (either $v$ is stochastic or $\bsigma(hh'v)$ is a randomised action), then we then have $\Lambda(hh'v) = \Lambda(h)$.
    Let $\{w_1, \dots, w_k\} = \Supp (\bsigma(hh'v))$. For brevity, let $\Bar{h}=hh'v$. 
    Then, either the sets $\Lambda(\Bar{h}w_1), \dots, \Lambda(\Bar{h}w_k)$ 
    \begin{itemize}
        \item  form a partition of $\Lambda(h)$, or
        \item $v$ is controlled by $i\in \Lambda(\Bar{h})$, and therefore $i \in \Lambda(\Bar{h}w_\l)$ for all $\l\in[k]$. 
    \end{itemize}
    It the latter case, if we consider two sets $\Lambda(\Bar{h}w_\l)$ and $\Lambda(\Bar{h}w_{\l'})$ with $\l \neq \l'$, they have exactly one element in common.
    That implies that any set of the form $\Lambda(\Bar{h}w_\l h'')$ that has cardinality at least $2$ is necessarily different from every set of the form $\Lambda(\Bar{h}w_{\l'} h'')$ with $\l' \neq \l$.
    And, therefore, that we have $f(h) = \sum_\l f(\Bar{h}w_\l)$.

% \thejaswini{I think this proof has too many components of reasoning about the sizes of the sets, and also about the shape of the sets simultaneously. We need to distil the combinatorics from the strategy shape. I would recommend some lemma/proposition/claim as above~\cref{lemma:counting_subset_dag}, and then just showing that the $\Lambda(v)$-compatible sets have a DAG structure described before.}
    
    % Splits occur when a stochastic node is visited, or when some player proceeds to a randomized action: if $\bsigma_{\|h}$ is fully deterministic (pure and visiting no stochastic vertex), then only the set $\Lambda(h)$ has the desired form, hence we have $f(h) = 1 < 3m-3$ and the proof is done.
    % Otherwise, let $h'$ be the shortest history such that $hh'$ is compatible with $\bsigma$, and that $\bsigma(hh')$ is a random transition: we then have $\Lambda(hh') = \Lambda(h)$.
    % Let $\{w_1, \dots, w_k\} = \Supp (\bsigma(hh'))$.    
    % Then, the sets $\Lambda(hh'w_1), \dots, \Lambda(hh'w_k)$ form a partition of $\Lambda(h)$, except for the case of the player controlling the last vertex of the history $hh'$, if there is any and if they belong to $\Lambda(h)$: that player would then be in each of those sets.
    % It is then still true that, if we consider two sets $\Lambda(hh'w_\l)$ and $\Lambda(hh'w_{\l'})$ with $\l \neq \l'$, they have at most one element in common.
    % That implies that any set of the form $\Lambda(hh'w_\l h'')$ that has cardinality at least $2$ is necessarily different from every set of the form $\Lambda(hh'w_{\l'} h'')$ with $\l' \neq \l$.
    % And, therefore, that we have $f(h) = \sum_\l f(hh'w_\l)$.
    
    If there is $\l$ such that $\Lambda(hh'w_\l) = \Lambda(hh') = \Lambda(h)$, then for every $\l' \neq \l$, the set $\Lambda(hh'w_{\l'})$ contains at most one element, hence $f(hh'w_{\l'}) = 0<3m-3$.
    But in such a case, we can extend $h'$ with $w_\l$ and the sequel, until we find a history $h'$ such that $hh'$ is compatible with $\bsigma$, that $\bsigma(hh')$ is a random transition, that $\Lambda(hh') = \Lambda(h)$ and that there is no $w_\l$ such that $\Lambda(hh'w_\l) = \Lambda(h)$ (if this process does not terminate, it means that $\Lambda(h)$ is actually never split, i.e. $f(h) = 1$, and the proof is done).
    Then, we can apply our induction hypothesis, and we obtain the inequality:
    $$f(h) \leq \sum_\l (3 |\Lambda(hh'w_\l)| - 3) = 3 \sum_\l |\Lambda(hh'w_\l)| - 3k.$$
    Let us now note that from the observation we made above about the sets $\Lambda(hh'w_\l)$, we can deduce the inequality $\sum_\l |\Lambda(hh'w_\l)| \leq m - 1 + k$ (each of the $m$ elements of $\Lambda(h)$ occurs once in these sets, except maybe one that may occur $k$ times).
    Hence:
    $$f(h) \leq 3 (m - 1 + k) - 3k = 3m - 3,$$
    as desired.
    \end{claimproof}
%    To do so, for each history $h$, let $f(h)$ be the number of sets of the form $\Lambda(hh')$ that has cardinality at least $2$, where $h'$ is a history; and let us prove that if $|\Lambda(h)| = m > 0$ then we have $f(h) \leq 3m-3$.

    Thus, if we take $h = v_0$, we find that there exist at most $3p-3$ sets of the form $\Lambda(v_0 h')$ with cardinality at least $2$.
    If we add all the singletons and the empty set, there are, then, at most $4p-2$ sets of the form $\Lambda(v_0 h')$, and therefore $4np-2n$ states of the form $\anchor_{Pv}$.
    If we add the states of the form $\punish_i$ and the state $\anchor_{\Pi\bot}$, we have in total at most $4np-2n+p+1$ states, as desired.


    \paragraph*{Definition of the strategy profile $\bsigma^\star$}

    We now have the states of our Mealy machine, let us define the transitions.\theju{what Mealy machine? Need to say that strategies are in the form of a Mealy machine, maybe?}
    First, let us define what $\sigma^\star$ does when in state $\punish_i$, for some player $i$: those states will correspond to the \emph{punishing strategies}, followed when player $i$ deviates.
    By Lemma~\ref{lm:reach_safe_positional}, there is a positional strategy profile $\btau^{\dag i}_{-i}$ that minimizes, from every vertex of the game, the payoff that player $i$ can enforce.
    Let us pick an arbitrary positional strategy $\sigma^{\dag i}_i$.
    Then, when the strategy profile $\bsigma^\star$ is in memory state $\punish_i$ and reads the vertex $v$, it outputs the action $\btau(v)$ and stays in state $\punish_i$.
    
    Let us now define what happens in state $\anchor_{\emptyset v}$.
    Consider the Boolean objective of achieving a payoff vector that has nonzero probability to be achieved in $\bsigma$, and avoiding every vertex that has probability zero of being visited in $\bsigma$.
    By Lemma~\ref{lm:reach_safe_positional}, there exists a positional strategy profile that is uniformly optimal for that objective: let us call it $\btau^{\anch \emptyset}$.
    Then, when in memory state $\anchor_{\emptyset v}$ and reading the vertex $w$, we distinguish two cases:
    \begin{itemize}
        \item if $vw$ is an edge that is compatible with the strategy profile $\btau^{\anch \emptyset}$, then the strategy profile $\bsigma^\star$ outputs the action $\btau^{\dag i}$, where $i$ is the player controlling $v$, and shifts to the memory states $\punish_i$;

        \item otherwise, it outputs the action $\btau^{\anch \emptyset}(w)$ and moves to the memory state $\anchor_{\emptyset w}$.
    \end{itemize}

    We can now move to singletons, and define what happens in the states of the form $\anchor_{\{i\} v}$.
    In that state, our objective is to give player $i$ exactly the risk entropy $z_i$.
    More precisely, consider the objective where player $i$ receives payoff $z_i$ with non-zero probability and ensuring that no vertex that has zero probability of being visited in $\bsigma$ is visited.\theju{should we say something about strategy restricted to the history?}    
%    of giving, with nonzero probability, the payoff $z_i$ to player $i$, and maintaining to $0$ the probability of achieving a payoff vector (including $0$ for every player) that has probability zero to be achieved in $\bsigma$, or of visiting a vertex that has probability zero to be visited in $\bsigma$. 
    By Lemma~\ref{lm:reach_safe_positional}, there exists a positional strategy profile $\btau^{\anch \{i\}}$ that satisfies that objective from every vertex from which it is possible.
    Note that that objective is in particular satisfiable, and therefore satisfied by $\btau^{\anch \{i\}}$, from every vertex $v$ such that there exists a history $hv$ compatible with $\bsigma$ such that $i \in \Lambda(hv)$.
    Similar to the previous step, we define the strategy profile $\bsigma^\star$ in the states of the form $\anchor_{\{i\} v}$ so that it follows the strategy profile $\btau^{\anch \{i\}}$, remembers the last vertex that was visited and use that memory to switch to the corresponding punishing state when some player $j$ deviates.

    Now, let us consider the states of the form $\anchor_{P v}$, where $P$ has cardinality at least $2$.
    The existence of $\anchor_{P v}$ implies that there is a history $h$ such that $\Lambda(h) = P$.
    Moreover, since each randomization splits the label of histories in sets that have at most one element in common, there is only one side of each split that can contain $P$, which implies that there is such a history that is minimal for the prefix relation --- we therefore choose that one.
    After $h$, the histories labelled by $P$ form a (possibly empty) sequence $hv_1, hv_1v_2, \dots$ which may be infinite, or ends with a new split.
    

    Let us first consider the finite case: there is, then, a longest history $hv_1 \dots v_q$ with $\Lambda(hv_1 \dots v_q) = P$.
    Then, there are at least two vertices $w_1, \dots, w_k \in \Supp(\bsigma(hv_1 \dots v_q))$ such that $\Lambda(hv_1 \dots v_q w_\l) \neq \emptyset$ for each $\l$.
    Therefore, the strategy profile $\bsigma_{\|h}$ guarantees, from the vertex $\last(h)$, that the vertex $v_q$ is reached with nonzero probability.
    By Lemma~\ref{lm:reach_safe_positional} (and by replacing $v_q$ by a terminal), there exists then a positional strategy profile that satisfies that requirement: let us write it $\btau^{\anch P}$.
    Let then $h'v_q$ be a simple history from $\last(h)$ to $v_q$ that is compatible with the strategy profile $\btau^{\anch P}$.
    We define the strategy profile $\bsigma^\star$ in each state $\anchor_{Pv}$ so that it follows the strategy profile $\btau^{\anch P}$ and remembers the last vertex visited, and switches to the state $\punish_i$ and follows the strategy profile $\btau^{\dag i}$ when a given player $i$ deviates and takes an edge that they are not supposed to take.
    Moreover, when an edge is taken that does belong to the history $h'v_q$, but not because a player deviated (it is then necessarily because of a stochastic node), the strategy profile switches to the corresponding state $\anchor_{\emptyset v}$ and immediately follows the corresponding strategy.
    Finally, when the vertex $v_q$ is reached when in state $\anchor_{P \last(h')}$, the strategy profile $\bsigma^\star$ chooses randomly between the edges $v_q w_1$, \dots, and $v_q w_k$.



    Let us finally consider the infinite case: then, the set $P$ is never split, except possibly into $\emptyset$ or some singleton $\{i\}$ and the set $P$ itself.
    There is, therefore, a play $\pi$ such that for every $k \geq 0$, we have $\Lambda(h\pi_{< k}) = P$.
    And, by the induction hypothesis maintained during the construction of $\Lambda$, for each optimistic $i \in P$, we have $\re_{\bsigma_{\|h\pi_{<k}}}[\mu_i] = z_i$; and for each pessimistic $i \in P$, the strategy profile $\bsigma_{-i\|h\pi_{<k}}$ is such that whatever player $i$ plays, they get a risk entropy at most $z_i$\dots which means that in the strategy profile $\bsigma_{\|h\pi_{<k}}$ itself, such a pessimist $i$ gets at most the risk entropy $z_i$; and in fact, exactly $z_i$, otherwise their risk entropy in $\bsigma$ would be lesser than $z_i$.
    We can then show that for each $i \in P$, we actually have $\mu_i(h\pi) = z_i$ and $\prob_{\bsigma_{\|h}}(\pi) \neq 0$\footnote{Note that this result is actually almost immediate when $\pi$ reaches a terminal; the arguments we present here are designed to include also the case where it does not, and therefore where we actually have $z_i = 0$ for all $i$.}.
    Indeed, let us recall that in the construction of $\Lambda$, when there were several possibilities for the set to which a given player could be added, we always favoured the empty ones: that means that, for each $k$, the vertex $\pi_{k+1}$ was actually the only element of $\Supp(\bsigma(h\pi_{<k}))$ satisfying the required properties.
    Consider then the two cases:

    \begin{itemize}
        \item If $i$ is an optimist: then, by the induction hypothesis maintained during the construction of $\Lambda$, we have $\re_{\bsigma_{\|h}}[\mu_i] = z_i$, and therefore $\prob_{\bsigma_{\|h}}(\mu_i = z_i) > 0$, i.e.:
        $$\sum_k \sum_{w \in E(\pi_k) \setminus \{\pi_{k+1}\}} \prob_{\bsigma_{\|h}}(\pi_{\leq k} w) \prob_{\bsigma_{\|h}}(\mu_i = z_i \mid \pi_{\leq k}w) + \prob_{\bsigma_{\|h}}(\pi) \prob_{\bsigma_{\|h}}(\mu_i \mid \pi) > 0.$$
        But by the remark made above, all the terms of the left sum are zero, hence we actually have $\prob_{\bsigma_{\|h}}(\pi) \prob_{\bsigma_{\|h}}(\mu_i \mid \pi) > 0$, i.e. $\prob_{\bsigma_{\|h}}(\pi) > 0$ and $\mu_i(\pi) = z_i$.

        \item If $i$ is a pessimist, then because of that same remark, for every $k \geq 0$ and each $w \in \Supp\left(\bsigma\left(h\pi_{\leq k}\right)\right)$, there exists a strategy $\tau_i^{kw}$ such that $\re_{\bsigma_{-i\|h\pi_{\leq k}w}, \tau_i^{kw}}[\mu_i] > z_i$.
        By composing all those strategies, we obtain a deviation $\tau_i$ of the strategy $\sigma_{i\|h}$; which, by the induction hypothesis maintained during the construction of $\Lambda$, satisfies the inequality $\re_{\bsigma_{-i\|h}, \tau_i}[\mu_i] \leq z_i$, i.e. either $\prob_{\bsigma_{-i\|h}, \tau_i}(\pi) = \prob_{\bsigma_{\|h}}(\pi) \neq 0$ and $\mu_i(\pi) \leq z_i$ (and then actually $\mu_i(\pi) = z_i$), or:
        $$\min_k \min_{w \in \Supp\left(\bsigma\left(h\pi_{\leq k}\right)\right) \setminus \{\pi_{k+1}\}} \re_{\bsigma_{-i\|h\pi_{\leq k}w}, \tau^{kw}_i}[\mu_i] \leq z_i,$$
        which is impossible by definition of the strategies $\tau_i^{kw}$.
    \end{itemize}

    Then, since $\pi$ has nonzero probability to be achieved, it traverses finitely many stochastic nodes.
    We can therefore define a lasso $\pi^\star$ with $\pi^\star_0 = \pi_0$, $\Occ(\pi^\star) = \Occ(\pi)$ and $\mu(\pi^\star) = \mu(\pi)$, which also traverses finitely many stochastic nodes.
    Then, we can define $\sigma^\star$ in the states of the form $\anchor_{P v}$ as following the positional strategy profile $\btau^P$, which follows deterministically the play $\pi^\star$, and remembering the last vertex seen.
    Then, when a player $i$ deviates and takes an edge that should not be taken, it switches to the strategy profile $\btau^{\dag i}$ and the state $\punish_i$.
    Finally, when an edge is taken that does not belong to $\pi^\star$ but does not correspond to a deviation either, we switch to the state $\anchor_{\emptyset w}$, with the last visited vertex $w$, and to the corresponding strategy profile.

    Let us end by the initialization: the strategy profile $\bsigma^\star$ initializes in the state $\anchor_{\Pi\bot}$.
    In this state, it behaves exactly as in any state of the form $\anchor_{\Pi v}$, but without having memorized a last visited vertex $v$, since there is no such vertex.
    From that state therefore, it necessarily reads the vertex $v_0$, proceeds to the action $\btau^{\anch \Pi}(v_0)$, and switches to the memory state $\anchor_{\Pi v_0}$, unless $v_0$ is already the vertex that the strategy profile $\btau^{\anch \Pi}$ aims at reaching, in which case it proceeds immediately to the corresponding split.


    % \paragraph*{The strategy profile $\bsigma^\star$ has the desired risk entropies.}
\begin{proposition}
    Let $\bsigma^\star$ be a strategy as constructed above from a risk sensitive equilibrium $\bsigma$. Then for each player $i$, $\re_{\bsigma^\star}[\mu_i] = z_i$.
\end{proposition}
\begin{claimproof}
    
    Let $i$ be a player: we want to prove that $\re_{\bsigma^\star}[\mu_i] = z_i$.
    Let us first see how $z_i$ is achieved in the strategy profile $\bsigma$: let $P \subseteq \Pi$ be the smallest set containing $i$ such that there exists a history $h$ with $\Lambda(h) = P$.
    Then, by construction of $\Lambda$, there exists a finite sequence of sets $\Pi = P_0, P_1, \dots, P_m = P$ and of histories $h_1 v_1 w_1, \dots, h_m v_m w_m$ where for each $k$, the history $h_{k+1}$ starts from $w_k$, the history $h_1 v_1 \dots h_k v_k w_k$ is compatible with $\bsigma$, and we have $\Lambda(h_1 v_1 \dots h_k v_k) = P_{k-1}$ and $\Lambda(h_1 v_1 \dots h_k v_k w_k) = P_k$.
    The strategy profile $\bsigma^\star$ follows initially the positional strategy profile $\btau^{\anch \Pi}$, from the vertex $v_0$: with non-zero probability, that strategy profile generates a history $h'_1 v_1$ from $v_0$ to $v_1$.
    From that vertex, it proceeds to a randomized action and, with nonzero probability, moves to the vertex $w_1$ and switches to the positional strategy profile $\btau^{\anch P_1}$, and so on: there is, therefore, a history $h'_1 v_1 h'_2 v_2 \dots h'_m v_m w_m$ that is compatible with the strategy profile $\bsigma^\star$ and after which $\bsigma^\star$ is in the state $\anchor_{P v_m}$, and plays accordingly.

    Then, we are in the case where the set $P$ is no longer split: there is an infinite play $\pi$ from $w_m$ such that $\Lambda(h_1 v_1 \dots h_m v_m \pi_{\leq k}) = P$ for every $k$.
    Then, in the construction of the strategy profile $\bsigma^\star$ we have distinguished two cases: the one where $P$ was a singleton, and the one where it had at least two elements (the empty case is excluded, since $P$ contains the player $i$).
    But in both cases, the strategy profile $\bsigma^\star$ follows the strategy profile $\btau^{\anch P}$ which, with nonzero probability, achieves the payoff $z_i$.
    
    Therefore, the strategy profile $\bsigma^\star$ is such that, with some nonzero probability, player $i$ gets the payoff $z_i$.
    We still have to prove that that player has zero probability of getting a lower payoff (if they are a pessimist) or a higher payoff (if they are an optimist).
    In both cases, that will be the case if we prove that any payoff vector $\bz'$ that has nonzero probability to be achieved in $\bsigma^\star$ had also nonzero probability to be achieved in $\bsigma$.
    Let therefore $\bz'$ be such a payoff vector\footnote{Again, the arguments that follow are actually necessary only because of the case in which $\bz'$ is the zero vector, obtained when no terminal is reached: the case where it corresponds to a terminal could simply be handled by noticing that $\bsigma^\star$ visits only vertices, including the terminals, that have nonzero probability to be visited in $\bsigma$.}.
    Then there is a history $hw$ compatible with $\bsigma^\star$ and a set $P \subseteq \Pi$ such that, after the history $hw$, the strategy profile $\bsigma^\star$ is in state $\anchor_{P \last(h)}$, and from that point, has non-zero probability of achieving payoff vector $\bz'$ while staying in states of the form $\anchor_{P v}$.
    If $P = \emptyset$, then the strategy profile $\btau^{\anch \emptyset}$ has been defined as a uniformly optimal strategy profile for the objective of realizing a payoff vector that has nonzero probability to be achieved in $\bsigma$.
    That objective is achievable, and therefore achieved by $\btau^{\anch \emptyset}$, from the vertex $w$, since that vertex is reached with nonzero probability in the strategy profile $\bsigma$.
    Therefore, the payoff vector $\bz'$ is also achieved with nonzero probability in $\bsigma$.
    If $P$ is a singleton $P = \{j\}$, then similarly, the strategy profile $\btau^{\anch \{j\}}$ has been defined as a strategy profile that is uniformly optimal\theju{what does uniformly optimal mean? I think I missed it} for an objective satisfiable from $w$ that includes avoiding the payoff vectors that have probability $0$ to be achieved in $\bsigma$: therefore, again, the payoff vector $\bz'$ is also achieved with nonzero probability in $\bsigma$.
    If now $P$ has at least two elements, then the strategy profile $\bsigma^\star$ stays in states of the form $\anchor_{P v}$ only along one play, which generates a payoff vector that was also associated with a play that has nonzero probability to be generated in $\bsigma$, hence the same conclusion.
\end{claimproof}

\begin{proposition}
    The strategy profile $\bsigma^\star$ constructed as above is a risk sensitive equilibrium
\end{proposition}
\begin{claimproof}
    We show that no player has an incentive to deviate, and deal with the cases 
    of a player being an optimist or a pessimist. 
    \paragraph*{No optimist has a profitable deviation in $\bsigma^\star$.}

    Let $i$ be an optimist, and let us assume that player $i$ has a profitable deviation from $\bsigma^\star$, i.e. that there is a strategy $\sigma'_i$ of player $i$ such that the strategy profile $(\bsigma^\star_{-i}, \sigma'_i)$ achieves with nonzero probability a payoff strictly greater than $z_i$.

    Let us notice that along every play compatible with $\bsigma^\star_{-i}$, the strategy profile $\bsigma^\star$ can have transitions among states of the form $\anchor_{P v}$ for a fixed $P$, from a state of the form $\anchor_{P v}$ to a state of the form $\anchor_{Q w}$ with $Q \subset P$, from a state of the form $\anchor_{P v}$ to the state $\punish_i$, or from $\punish_i$ to itself.
    Therefore, any such play stabilizes either in the state $\punish_i$, or among the states of the form $\anchor_{P v}$ for a fixed set $P$.
    Consequently, if in the strategy profile $(\bsigma^\star_{-i}, \sigma'_i)$ player $i$ gets a payoff greater than $z_i$ with nonzero probability, then we can also say that either:
    \begin{itemize}
        \item with nonzero probability, player $i$ gets such a payoff \emph{and} the state $\punish_i$ is reached;

        \item or with nonzero probability, player $i$ gets such a payoff and there exists $P \subseteq \Pi$ such that the strategy profile $\bsigma^\star_{-i}$ remains in states of the form $\anchor_{P v}$.
    \end{itemize}

    The first case is impossible: for any history $hv$ compatible with $\bsigma^\star_{-i}$ such that that strategy profile is in an anchoring state after $h$ and in state $\punish_i$ after $hv$, we have that the vertex $\last(h)$ is also visited with nonzero probability in the strategy profile $\bsigma$.
    Then, if by moving to $v$ player $i$ can get with nonzero probability a payoff greater than $z_i$ against the strategy profile $\bsigma^\star_{-i\|hv} = \btau^{\dag i}_{-i}$, then they can do so against every strategy profile, which induces a profitable deviation in the $\brho$-RSE $\bsigma$.

    As for the second case, let us notice that the strategy profiles of the form $\btau^{\anch P}$ are pure, and therefore that any deviation of player $i$ is immediately detected and leads to a switch to state $\punish_i$.
    Therefore, if $\bsigma^\star$ remains in states of the form $\anchor_{P v}$, it means that player $i$ is actually following the strategy $\sigma^\star_i$, which cannot be a profitable deviation.


    \paragraph*{No pessimist has a profitable deviation.}

    Let $i$ be a pessimist, and let us assume that $i$ has a profitable deviation, i.e. that there exists a strategy $\sigma'_i$ such that in the strategy profile $(\bsigma^\star_{-i}, \sigma'_i)$, it is almost sure that player $i$ will get no payoff lesser than or equal to $z_i$.

    First, let us notice that for each history $hv$ compatible with $\bsigma^\star$ such that, after $hv$, the strategy profile $\bsigma^\star$ is in state $\anchor_{P \last(h)}$ with $i \in P$, the vertex $v$ is such that there also exists a history $h'v$ compatible with $\bsigma$ and such that $\Lambda(h'v) = P$, and by the induction hypothesis maintained during the construction of $\Lambda$, we have $\re_{\bsigma_{-i\|h'v}, \tau_i}[\mu_i] \leq z_i$ for every $\tau_i$.
    Therefore, if, from $v$, player $i$ takes an edge that makes $\bsigma^\star_{-i}$ switch to the state $\punish_i$, then with nonzero probability player $i$ gets a payoff lesser than or equal to $z_i$.
    If $\sigma'_i$ is a profitable deviation, such an action is therefore never performed.

    Then, since for every history $hv$ such that the strategy profile $\bsigma^\star$ is in state $\anchor_{P \last(h)}$ and $\bsigma^\star(h)$ is a randomized action, there is at least one $w \in \Supp(\bsigma^\star(hv))$ such that $\bsigma^\star$ is in state $\anchor_{Q v}$ with $i \in Q$ after $hvw$; and that is the case of every $w \in \Supp(\bsigma^\star(hv))$ if $v \in V_i$.
    Thus, if the strategy $\sigma'_i$ observes the constraint described above, there still exists a set $P$ with $i \in P$ such that, with nonzero probability, when following the strategy profile $(\bsigma^\star_{-i}, \sigma'_i)$, the strategy profile $\bsigma^\star_{-i}$ stabilizes among memory states of the form $\anchor_{P v}$, and therefore follows the strategy profile $\btau^{\anch P}_{-i}$.
    Moreover, since the strategy profile $\btau^{\anch P}$ is positional, player $i$ must follow the strategy $\tau^{\anch P}_i$, otherwise any other action would lead to a switch to the state $\punish_i$.
    But then, by definition of the strategy profile $\btau^{\anch P}$, player $i$ gets the payoff $z_i$ with nonzero probability, and the deviation is not profitable.
    \end{claimproof}
    The strategy profile $\bsigma^\star$ is a $\brho$-RSE, satisfies the equality $\re_{\bsigma^\star}[\mu] = \re_{\bsigma}[\mu]$, and uses the desired number of memory states.
\end{proof}



\begin{theorem}
    The constrained existence problem of $\brho$-RSEs is $\NP$-complete.
\end{theorem}

\begin{proof}
    The lower bound is given by~\cref{lm:infinite_rho_np_hardness}.

    Now, let $\Game_{\|v_0}$ be a simple quantitative stochastic game, let $\brho$ be a risk-sensitivity vector with only infinite values, and let $\bx$ and $\by$ be threshold vectors.
    By \cref{lm:rse_finite_memory}, if there exists a $\brho$-RSE with $\bx \leq \re_\bsigma[\mu] \leq \by$, there exists one with at most $4np-2n+p+1$ memory states, where $p$ is the number of players and $n$ is the number of vertices.
    Such a strategy profile can be guessed in polynomial time.
    
    We now need to show that it can be checked in polynomial time.
    That can be done as follows:
    \begin{itemize}
        \item First, compute the vector $\re_\bsigma[\mu]$: by \cref{lm:mpd_ptime}, that can be done in polynomial time, by computing the corresponding risk entropies in the Markov chain induced by $\bsigma$ (which has polynomial size).

        \item Second, check that $\bx \leq \re_\bsigma[\mu] \leq \by$.
        That can clearly be done in polynomial time.

        \item Third, check for each player $i$ that player $i$ has no profitable deviation: by ~\cref{lm:mpd_ptime}, that can be done in polynomial time by computing the best risk entropy player $i$ can get in the MDP induced by $\bsigma_{-i}$ (which has polynomial size).
    \end{itemize}
\end{proof}

\leonard{I no longer believe in FPTness: we also need to find the vertices in which the splits occur, and that requires a time exponential in the number of vertices...}

\begin{theorem}\label{thm:infinite_rho_restricted_strategy_np_easy}
    The constrained existence problem of $\brho$-RSEs is $\NP$-complete
    \theju{, and fixed-parameter tractable?} 
    when the number of players is fixed, even when the players are restricted to positional, memoryless,  or pure strategies. 
\end{theorem}
\begin{proof}
    The lowerbound for all three of the above cases follow from \cref{cor:np_hardness_restricted_strat}. 
        \thejaswini{This is not a proof. A proof sketch only.}
    For the upper bound, we show that we can still guess a strategy and verify in polynomial time if it is indeed a strategy. For the cases of positional and memoryless strategies, guessing a strategy is straightforward. Whereas for pure strategies, this requires some work. 
    \paragraph*{Positional strategies and memoryless strategies} The size of such a strategy $\sigma$ that is an RSE can be represented using polynomially many bits, since one only needs to guess the set of edges from each vertex that are being used with non-zero probability. From \cref{lm:mpd_ptime}, we can then verify if the given $\sigma$ indeed gives a simple quantitative payoff within the constraints, and also if it is indeed an RSE in polynomial time. 

    \paragraph*{Pure strategies}
    For pure strategies, the strategies might require more memory to represent. We argue therefore that if there is a winning strategy, there is one that requires only 
\end{proof}
